Locality-Preserving Hashing for Shifts with Connections to Cryptography

Can we sense our location in an unfamiliar environment by taking a sublinear-size sample of our surroundings? Can we efficiently encrypt a message that only someone physically close to us can decrypt? To solve this kind of problems, we introduce and study a new type of hash functions for finding shifts in sublinear time. A function $h:\{0,1\}^n\to \mathbb{Z}_n$ is a $(d,\delta)$ {\em locality-preserving hash function for shifts} (LPHS) if: (1) $h$ can be computed by (adaptively) querying $d$ bits of its input, and (2) $\Pr [ h(x) \neq h(x \ll 1) + 1 ] \leq \delta$, where $x$ is random and $\ll 1$ denotes a cyclic shift by one bit to the left. We make the following contributions. * Near-optimal LPHS via Distributed Discrete Log: We establish a general two-way connection between LPHS and algorithms for distributed discrete logarithm in the generic group model. Using such an algorithm of Dinur et al. (Crypto 2018), we get LPHS with near-optimal error of $\delta=\tilde O(1/d^2)$. This gives an unusual example for the usefulness of group-based cryptography in a post-quantum world. We extend the positive result to non-cyclic and worst-case variants of LPHS. * Multidimensional LPHS: We obtain positive and negative results for a multidimensional extension of LPHS, making progress towards an optimal 2-dimensional LPHS. * Applications: We demonstrate the usefulness of LPHS by presenting cryptographic and algorithmic applications. In particular, we apply multidimensional LPHS to obtain an efficient "packed" implementation of homomorphic secret sharing and a sublinear-time implementation of location-sensitive encryption whose decryption requires a significantly overlapping view.

==> 2D-LPHS.tex <==
% !TEX root = ../LPHS.tex

\section{Multi-Dimensional LPHS}\label{sec:2dim}
%\subsection{Old stuff}
%
%In this section, we analyze the 2-dimensional LPHS.
%
%Once again, the goal is to understand how $\delta$ behaves as a function of the other parameters $(n,b,d,\eps)$ for 2DLPHS in terms of upper bounds and lower bounds. Below, we give some initial results for the specific case of $\eps = 0$ (i.e., noiseless 2DLPHS).
%
%\subsubsection{Lower Bound}
%
%\begin{theorem}
%	\label{thm:lower2}
%	For any $(n,1,d,0,\delta)$-2DLPHS,
%	$$\delta = \Omega(1/d).$$
%\end{theorem}
%The proof of Theorem~\ref{thm:lower2} is a generalization of the lower bound proof for noiseless (standard) LPHS. It is obtained by using the bound
%$$
%\pr_{x^{(2,b)},r_1 \sim U(0, d),r_2 \sim U(0, d)} \lbs h(x^{(2,b)}) \neq h(y^{(2,b)} \ll (r_1,r_2)) + (r_1,r_2) \rbs
%= \Omega(1),$$
%which is derived based on (birthday type) arguments, similar to those used for proving the lower bound for noiseless standard LPHS (since a $d \times d$ square contains $d^2$ points). Then, Theorem~\ref{thm:lower2} follows from a triangle inequality (union bound).
%
%\subsubsection{Upper Bound}
%
%\begin{conjecture}\label{conj:upper2}
%	There is an $(n,1,d,0,\delta)$-2DLPHS that satisfies $\delta = \tilde{O}(1/d)$,
%	where $\tilde{O}$ hides a logarithmic factor in $d$.
%\end{conjecture}
%We propose an algorithm (i.e., a function $h$) that is a variant of the iterated random walk described in~\cite{DKK18}. We have $I$ iterations, where $I \approx \log\log d$, and each iteration has about $d$ steps (we allow the algorithm about $d \log\log d$ steps in total).
%
%In iteration $i \in \{1,2,\ldots,I\}$, we set $m_i = d^{1/2 - 2^{-i}}$ (i.e. $m_i = 1,d^{1/4},d^{3/8},d^{7/16},\ldots,\approx d^{1/2})$.
%In each step, according to the value of the current position $(x,y)$, we move to $(x + a, y + b)$, where $a,b$ are integers in the interval $[-m_i, m_i]$, selected independently (and uniformly) according to the current position (by applying a PRF). As in the original iterated random walk, at the end of each iteration, we move to the position with the minimal encountered value (the value of each location is determined by a PRF). The algorithm outputs the $(x,y)$ distance of its final location from its initial position.
%
%For the analysis, we assume that we have two parties initially located on a 2-dimensional grid at distance 1 on either the $x$ or the $y$ axis. Each party independently applies the above algorithm. We analyze the probability that the parties' walks coincide (i.e., the parties meet) during the algorithm, which implies that the algorithm succeeds. The analysis is based on the  following claims.
%\begin{enumerate}
%	\item At the beginning of iteration $i$, given that the parties did not meet yet, their expected distance is $O((m_i)^2)$ in each coordinate.
%	\item Given that the parties have not met up to iteration $i$, the expected number of steps (of both) until they collide in iteration $i$ is $O(m_i \cdot d^{1/2})$.
%\end{enumerate}
%Roughly, the second claim implies that the probability that the parties do not meet at iteration $i$ (assuming they have not met previously) is $O(d \cdot (m_i \cdot d^{1/2})^{-1}) = O(d^{2^{-i}})$.
%Thus, the failure probability of the parties after all $I$ iterations is $\tilde{O}(1/d)$, as required.
%
%For the first claim, observe that the variance of the distance that each party moves in each coordinate in a step of iteration $i$ is $(m_i)^2$, hence the total variance after $d$ steps is $d \cdot (m_i)^2$. Hence, the expected distance after iteration $i$ is $d^{1/2} \cdot m_i = d^{1 - 2^{-i}} = (m_{i+1})^2$ as required.
%
%The second claim requires a careful analysis of the random walk. One obstacle that requires handling is that the algorithm may run into a cycle in an iteration and waste the rest of its steps. This can be handled by defining a deterministic way of breaking cycles (e.g., by exiting through a point with a minimal value). Note that it is also possible to have several levels of cycles (e.g., a bigger cycle that contains smaller cycles, etc.). cycles are likely to complicate the analysis.

%In this section we study 2-dimensional LPHS (2D-LPHS) algorithms. First, we consider the `upper bound' side.
%, or 2D-LPHS for short.

%\ynote{What about non-cyclic? Also, should either make notation and terminology in this section consistent with the definitions, or explicitly say that we change notation. }
%\ohad{I commented about the first, and fixed the second.}


%\subsection{Setting}\label{ssec:2Dsetting}
%The input of a (possibly probabilistic) 2D-LPHS is a 2D-string $x \in \Sigma_b^{\integers_{n} \times \integers_{n}}$ for some `large' integers $b,n$
%\ynote{Why is $b$ large? Isn't it enough for $b$ to be logarithmic in $n$?} (which are implicitly passed as an input), and a `small' number $d$.

%The goal of a 2D-LPHS $h$ is to query the input string $x$ on at most $d$ keys, and output a value in $\integers_{n} \times \integers_{n}$, so that

In this section we study the $k$--dimensional generalization of LPHS, focusing mainly on the case $k=2$ (2D-LPHS). First, in Section~\ref{sec:sub:upper}, we consider the upper bound side. We start with simple constructions achieving error $\delta=\tilde{O}(d^{-1/2})$ (Section~\ref{sec-simple}) and $\delta=\tilde{O}(d^{-4/5})$ (Section~\ref{sec-lesssimple}). The latter makes a black-box use of the 1-dimensional IRW algorithm of~\cite{DKK18}.
%, that achieves error rate of $\delta=\tilde{O}(d^{-4/5})$. 
More concretely, for $n = \Omega(d^{6/5})$, any $b \geq 3 \log n$ and any $(r_1,r_2) \in \{0,1\} \times \{0,1\}$, we have
\begin{equation}\label{eq:2Dreq}
\pr_{x \in_R \Sigma_b^{\integers_{n} \times \integers_{n}}}\lbs h(x)-h(x \ll (r_1,r_2)) \neq (r_1,r_2) \rbs = O(d^{-4/5}).
\end{equation}
Since our specific construction only issues queries in a limited box of dimensions $O(d^{6/5}) \times O(d^{4/5})$ while $n = \Omega(d^{6/5})$, it gives both a cyclic and a non-cyclic LPHS with the same parameters.

This proves a weak version of Theorem~\ref{thm:2dupper}. In Section~\ref{app:2D78} we
 obtain the improved upper bound of Theorem~\ref{thm:2dupper} 
by presenting a more intricate algorithm that achieves error rate of $\delta=\tilde O(d^{-7/8})$. 
%In addition, we present there 
Finally, in Section~\ref{app:2Dopt} we present a heuristic algorithm that we {\em conjecture} to achieve the near-optimal error probability of $\delta=\tilde{O}(d^{-1})$.  
%(which, if true, matches our lower bound up to a logarithmic factor). 
This conjecture is supported by experimental evidence.
%Appendix~\ref{app:2D}.

In Section~\ref{sec:sub:lower} we study limitations of $k$-dimensional LPHS. We prove Theorem~\ref{thm:kdlower}, which for $k=2$ implies that the error probability of a 2D-LPHS must satisfy $\delta=\tilde{\Omega}(d^{-1})$.

%The quality of a 2D-LPHS is measured by how low the `error probability' $\delta$ is, as a function of $d$. There are other quality measures relevant for the implementation of a 2D-LPHS, such as cache-friendliness; we do not consider these in this section. Moreover, for simplicity, we assume $b,n$ are large enough with respect to $d$ (e.g. $b,n \geq d^2$), and do not investigate the (different) behavior of 2D-LPHS for small $n$. (Smaller $b$ does not change the problem much, see Lemmas~\ref{lem:bigger-alphabet}, \ref{lem:smaller-alphabet}.) \ynote{Again, not clear why $b$ should be so big. }

%We notationally restrict our analysis to cyclic LPHS (i.e. the input is $x \in \Sigma_b^{\integers_n \times \integers_n}$), although all results in this section transparently apply to non-cyclic ones with $n$ large enough ($n \geq \Omega(d)$).
%\ynote{The input in the non-cyclic case is in  $\Sigma_b^{[n]\times[n]}$ , the difference is in the interpretation of the shift operator. Since all of our applications for 2D LPHS (including packed HSS) require the non-cyclic variant, it might be better to just write the proof for the non-cyclic case (using the new $\lll$ notation for the non-cyclic shift operator). Or maybe before the final theorem statement (which refers to both cases) we can explain why the same proof applies to both cases.
%}

\subsection{Upper bounds on 2D-LPHS algorithms}
\label{sec:sub:upper}

We begin by describing a very simple 2D-LPHS algorithm called \textsc{Min-Hash} that is similar to the 1D-LPHS described in Algorithm~\ref{alg:basic}.

\subsubsection{A simple 2D-LPHS with error rate $\delta = O(d^{-1/2})$}
\label{sec-simple}

\medskip
\noindent
\textbf{Notation} All integer operations in algorithms within this section are assumed to be floored. For example, we write $x/y$ for $\lfloor x/y \rfloor$ and $\sqrt{n}$ for $\lfloor \sqrt{n} \rfloor$.
\begin{algorithm}\label{alg:2Dstage1}
	\Begin{
		\Return $\mathrm{arg\,min}_{i,j\in [0, \sqrt{d}]} \{x[i,j]\}$
	}
	\caption{\textsc{Min-Hash}$(x \in \Sigma_{b}^{\integers_{n}^2},d \in \pintegers)$}
\end{algorithm}

The following lemma describes the performance of \textsc{Min-Hash}. The proof is presented in Appendix~\ref{app:2D}.
\begin{lemma}\label{lem:min-hash-pr} For $n = \Omega(d^{1/2})$ and any $b \geq 3 \log n$ and $(r_1,r_2) \in \{0,1\} \times \{0,1\}$,
	\begin{equation}\label{eq:min-hashErr}
	\pr\lbs \textsc{Min-Hash}(x, d)-\textsc{Min-Hash}(x \ll (r_1, r_2) , d) \neq (r_1, r_2) \rbs = O(d^{-1/2}).
	\end{equation}
\end{lemma}

\subsubsection{An IRW-based 2D-LPHS with error rate $\delta = O(d^{-4/5})$}
\label{sec-lesssimple}

In this subsection we demonstrate how an 1D-LPHS may be used in order to construct a 2D-LPHS with $\delta = O(d^{-4/5})$. Let us recall the functionality of an optimal 1D-LPHS, mentioned in Corollary~\ref{corr:DKK18_1}.
% \emph{optimal} 2D-LPHS can be achieved using only black-box calls to an optimal 1D-LPHS.
%\ynote{Last sentence sounds too apologetic. Maybe just say that we give here the best black-box construction of 2D-LPHS from 1D-LPHS we are aware of? }
%Let us recall the functionality of an optimal 1D-LPHS, mentioned in Corollary~\ref{corr:DKK18_1}.
%\paragraph{Optimal 1D-LPHS rephrasing}

\medskip\noindent
\textbf{Optimal 1D-LPHS, rephrased.}
	For $b \geq 3 \log n$, there exists an algorithm $\textsc{optimal1D}\colon \Sigma_b^{\integers_n} \times \integers \to \integers_n$ with the following properties. If $n = \Omega(d^2)$, then
	\[
	\pr_x[\textsc{optimal1D}(x, d) - \textsc{optimal1D}( x \ll 1, d) \neq 1] < O(1/d^{2}).
	\]
	
\medskip

%In turns out that calling $\textsc{optimal1D}$ recursively results in a pretty good 2D-LPHS algorithm, called \textsc{Recursive-Hash}.
The 2D-LPHS construction is described in the \textsc{Recursive-Hash} algorithm (Algorithm~\ref{alg:2D45}). The algorithm works in two stages, beginning from an initial input $(j,i)$, first returning a column $i_1$ and then a row $j_1$. The column $i_1$ is located by a walk along the row $j$ which uses the \textsc{optimal1D} algorithm with $d/d'-1$ queries (for a parameter $d'$). A query in this algorithm on column $i_0$ is answered by the \textsc{rec1D} algorithm, which executes \textsc{optimal1D} with $d'$ queries on column $i_0$. After returning column $i_1$, the textsc{Recursive-Hash} algorithm runs the \textsc{optimal1D} algorithm along this column, from input row $j$ to return the output row $j_1$. 

Sketching the analysis (formalized in the proof of Lemma~\ref{lem:2D45}), observe that there are three possible sources of error in the algorithm. First, the values that \textsc{rec1D} returns on shared columns $i_0$ may not be identical. However, since the parties start at row distance of at most 1, the executions of \textsc{optimal1D} from $x[j,i_0]$ and $x[j+1,i_0]$ agree on the same symbol in column $i_0$, except with probability $O((d')^{-2})$. Thus, with probability $1 - O((d')^{-2}) \cdot d/d'$, the column values defined by the \textsc{rec1D} algorithm agree for all columns visited by both parties. 

The second source of error is that although the column values of shared columns are identical, the two parties do not converge to the same column. Since each party queries $d/d'$ columns, the probability for this event is $O((d/d')^{-2})$. The third source of error is that the execution of \textsc{optimal1D} on the agreed column fails on  $d'$  queries. The probability for this event is $O(d'^{-2}$. Hence the total error probability is $\delta = O((d')^{-2} \cdot d/d' + (d/d')^{-2})$. Choosing $d' = d^{3/5}$ gives $\delta = O(d^{-4/5})$.

\begin{algorithm}
	\Begin{
		Define $u \in \Sigma_b ^{\integers_n}$ by $u[j] \gets z[j,i_{0}]$\\
		$j_0 \gets \textsc{optimal1D}(u, d')$\\
		\Return $z[j_0 + 10 d'^{2},i_0]$
	}
	\caption{\textsc{rec1D}$(z \in \Sigma_b^{\integers_{n}^2},d' \in \pintegers, i_{0} \in \integers_{n})$}
\end{algorithm}
%\vspace*{-0.6cm}
\begin{algorithm}
	\label{alg:2D45}
	\Begin{
		$i_1 \gets \textsc{optimal1D}(i \mapsto \textsc{rec1D}(z,d^{3/5}-1,i), d^{2/5})$\\
		$j_1 \gets \textsc{optimal1D}(j \mapsto z[j,i_1], d^{2/5})$\\
		\Return $(j_{1}, i_{1})$
	}
	\caption{\textsc{Recursive-Hash}$(z \in \Sigma_b^{\integers_{n}^2},d \in \pintegers)$}
\end{algorithm}
\begin{lemma}\label{lem:2D45}
	For $n = \Omega(d^{6/5})$ and any $b \geq 3 \log n$ and $(r_1,r_2) \in \{0,1\} \times \{0,1\}$,
	\begin{equation*}\label{eq:Rec2DErr}
	\pr\lbs \textsc{Rec2D}(x, d)-\textsc{Rec2D}(x \ll (r_1,r_2), d) \neq (r_1, r_2) \rbs =  O(d^{-4/5}).
	\end{equation*}
\end{lemma}


\subsubsection{3-Stage-Hash: a 2D-LPHS algorithm with $\delta = \tilde O(d^{-7/8})$}\label{app:2D78}
%\ohad{If this subsection is not ready until submission, please remove it!}

%The algorithm \textsc{3-Stage-Hash}, presented in this section, achieves an error probability of $\delta = O(d^{-7/8})$. This algorithm is the simplest 2D-LPHS algorithm we know of which outperforms \textsc{Recursive-Hash}. By presenting it, we mainly wish to demonstrate that there exist 2D-LPHS which (provably) beat \textsc{Recursive-Hash}.
In this subsection we prove Theorem~\ref{thm:2dupper}, by presenting the algorithm \textsc{3-Stage-Hash} which achieves error rate of $\delta=\tilde{O}(d^{-7/8})$.
\textsc{3-Stage-Hash} is composed of 3 stages. The first is \textsc{Min-Hash} and we refer to the other two as \textsc{stage2} and \textsc{stage3}.

\begin{algorithm}\label{alg:2D3stage}
	\Begin{
		$(i_0, j_0) \gets \textsc{Min-Hash}(z,\ d/3)$\\
		$(i_1, j_1) \gets \textsc{stage2}(z,\ d/3,\ i_0 + 2\sqrt{d},\ j_0+2\sqrt{d})$\\
		$(i_2, j_2) \gets \textsc{stage3}(z,\ d/3,\ i_1 + 2d^{3/4},\ j_1+2d^{3/4})$\\
		\Return $(i_2, j_2)$
	}
	\caption{\textsc{3-Stage-Hash}$(z \in \Sigma_b^{\integers_n^2},d \in \pintegers)$}
\end{algorithm}
\begin{algorithm}\label{alg:stage2}
	\Begin{
		$L \gets \sqrt[4]{d'}$\\
		Let $\psi_{1}, \psi_{2} \colon \Sigma_b \to \integers_{L}$ be $\psi_{1}(t)=t\ \mathrm{mod}\,L$ and $\psi_{2}(t)=\lfloor t/L\rfloor\ \mathrm{mod}\,L$\\
		$P, P' \gets \es, \es$\\
		$i \gets i_0$\\
		\For{$s=1$ to $\sqrt{d'}$}{
			$j \gets j_0$\\
			\For{$t=1$ to $\sqrt{d'}$}{
				$P' \gets P' \cup \{(i,j)\}$\\
				$j \gets j + 1 + \psi_{1}(z[i, j])$
			}
			$i \gets i + 1 + \psi_{2}(\min_{p'\in P'}\{z[p']\})$\\
			$P, P' \gets P \cup P', \es$
		}
		\Return $\mathrm{arg\,min}_{p\in P}\{z[p]\}$
	}
	\caption{\textsc{stage2}$(z \in \Sigma_b^{\integers_n^2}, d' \in \pintegers, i_0 \in \integers_{n}, j_0 \in \integers_{n})$}
	\end{algorithm}
\begin{algorithm}
	\Begin{
		Let $\psi \colon \Sigma_{b} \to \{-d'^{3/8}, \ldots, d'^{3/8}\}$ be $\psi(t) = (t\ \mathrm{mod}\, (2d'^{3/8}+1))-d'^{3/8}$\\
		$P \gets \es$\\
		$(i,j) \gets (i_0, j_0)$\\
		\For{$s=1$ to $d'$}{
			$P \gets P \cup \{(i,j)\}$\\
			$(i,j) \gets (i+1, j + \psi(z[i,j]))$
		}
		\Return $\mathrm{arg\,min}_{p\in P}\{z[p]\}$
	}
	\caption{\textsc{stage3}$(z \in \Sigma_b^{\integers_n^2}, d' \in \pintegers, i_0 \in \integers_{n}, j_0 \in \integers_{n})$}
\end{algorithm}

\begin{lemma}\label{lem:2D78-err}
Let $2^b,n\geq d^4$, and $r_1,r_2 \in \{0,1\}$. Then,
	\begin{equation}\label{eq:2D78}
	\pr\lbs \textsc{3-Stage-Hash}(x, d)-\textsc{3-Stage-Hash}(y, d) \neq (r_1, r_2) \rbs < O(d^{-7/8}),
	\end{equation}

\end{lemma}
In order to prove Lemma~\ref{lem:2D78-err}, we need the following facts,
%which we prove later.
whose proofs are presented in Appendix~\ref{app:2D}.
\begin{lemma}\label{lem:geoms}
	Let $S_1, S_2, \ldots$ be a sequence of i.i.d. geometric random variables: $S_i \sim \mrm{Geom}(p)$. If $K$ is the minimal integer with $\sum_{k=1}^{K} S_k \geq r$,	then $\be[K] \leq rp+1$.
\end{lemma}

\begin{lemma}\label{lem:sparse_walks}
	Let $I_0, I_1, I_2, \ldots$ be a random walk with $I_{k+1}-I_{k}$ being i.i.d. variables distributed as the difference of two uniform $U(0, m)$ random variables, with $m \in \pintegers$. If $T$ is the minimal time with $I_T = 0$, then
	\[
		\be[\min(T, r)] \leq O\left( (m + I_0/m) \sqrt{r}\right).
	\]
\end{lemma}


\begin{proof}[of Lemma~\ref{lem:2D78-err} (sketch)]
	Let $(i_k^z, j_k^z)$ be the values computed as $(i_k, j_k)$ at $\textsc{3-Stage-Hash}(z, d)$, for $k \in \{0,1,2\}$ and $z \in \{x,y\}$. We say that $(i_k^x, j_k^x)$ and $(i_k^y, j_k^y)$ are synchronized if $(i_k^x, j_k^x) - (i_k^y, j_k^y) = (r_1, r_2)$. Observe that if $(i_k^x, j_k^x)$ and $(i_k^y, j_k^y)$ are synchronized, then so are $(i_{k+1}^x, j_{k+1}^x)$ and $(i_{k+1}^y, j_{k+1}^y)$. This is because each stage $k+1$ of $\textsc{3-Stage-Hash}(z,d)$ deterministically depends on values queried from $z$ with offset $(i_k^z, j_k^z)$, so that evaluations keep being aligned. Overall,
	\begin{align}
	\begin{split}
		\delta \ddd &\pr_{x,y,r_1,r_2}[\textsc{3-Stage-Hash}(x, d) - \textsc{3-Stage-Hash}(y, d) \neq (r_1,r_2)]
		\\
		&\leq
		\pr[(i_0^x, j_0^x) - (i_0^y, j_0^y) \neq (r_1, r_2)] \cdot
		\\
		&\cdot \prod_{k=1}^{2}\pr\left[\given{(i_k^x, j_k^x) - (i_k^y, j_k^y) \neq (r_1, r_2)}{(i_{k-1}^x, j_{k-1}^x) - (i_{k-1}^y, j_{k-1}^y) \neq (r_1,r_2)}\right].
	\end{split}
	\end{align}
	Hence, to bound $\delta$ it is sufficient to verify the following three claims:
	\begin{enumerate}
	\item $\pr[(i_0^x, j_0^x) - (i_0^y, j_0^y) \neq (r_1, r_2)]\leq O(1/\sqrt{d})$.
	\item $\pr\left[\given{(i_1^x, j_1^x) - (i_1^y, j_1^y) \neq (r_1, r_2)}{(i_0^x, j_0^x) - (i_0^y, j_0^y) \neq (r_1, r_2)}\right] \leq O(1/\sqrt[4]{d})$.
	\item $\pr\left[\given{(i_2^x, j_2^x) - (i_2^y, j_2^y) \neq (r_1, r_2)}{(i_1^x, j_1^x) - (i_1^y, j_1^y) \neq (r_1, r_2)}\right] \leq O(1/\sqrt[8]{d})$.
	\end{enumerate}
	\medskip\noindent \textbf{\textit{Claim 1)}} Follows from Lemma~\ref{lem:min-hash-pr}.
	
	\medskip\noindent \textbf{\textit{Claim 2)}}	
	Since $\textsc{Min-Hash}(z,d)$ scans a $\sqrt{d} \times \sqrt{d}$ area and outputs a point inside it, we are guaranteed that $|i_0^x-i_0^y| \leq \sqrt{d}+1$ and $|j_0^x-j_0^y| \leq \sqrt{d} + 1$. Because $\textsc{stage2}$ is fed with the output point of $\textsc{Min-Hash}$ shifted by $2\sqrt{d}$ in each axis, its queries do not overlap these of $\textsc{Min-Hash}$, and its performance is independent of the $\textsc{Min-Hash}$ phase. Moreover, $\textsc{stage2}$ can be modeled as a random walk on the $i$ axis, whose steps are integers uniformly distributed in $[1, \sqrt{d/3}]$, which are determined by some random walk on the $j$ axis. Denote by $I_1^x, \ldots, I_{\sqrt{d'}}^x$ and $I_1^y, \ldots, I_{\sqrt{d'}}^y$ the sequences of $i$'s observed by $\textsc{stage2}$ applied on $x$ and on $y$.
	
	In order to compute the probability that the outputs of $\textsc{stage2}(x, d')$ and $\textsc{stage2}(y, d')$ are not synchronized, it is sufficient (following the proof of Lemma~\ref{lem:min-hash-pr}) to count the number of queries that the two processes make, which are not shared. These queries can be classified into two categories: queries with non-shared $i$, and queries with shared $i$ and non-shared $j$. Our goal is to show each class contains on average $O(d'^{3/4})$ such queries, yielding the probability of the outputs not being synchronized is $O(d'^{3/4}/d')$ (similarly to Lemma~\ref{lem:min-hash-pr}).
	We start by reasoning about the first class of queries, and then proceed to the second.
	
	Let $U_1$ denote the total number of $i$-steps until $i^x$ and $i^y$ are synchronized (i.e. $U_1 = k+k'$ when $k,k'$ are minimal with $I_k^x-I_{k'}^y=r_1$). Up to this point, the two $\textsc{stage2}$ applications act independently, as their queries do not overlap. Using~\cite[Lemmas 3,5]{DKK18} with $b \leq \sqrt{d}+1$ and $L=\sqrt[4]{d'}$ we see $\be[U_1] \leq O(d^{1/4})$. Next, we note that once $I_k^x-I_{k'}^y=r_1$, it is likely that $I_{k+1}^x-I_{k'+1}^y=r_1$. Specifically, we will show
	\[
		\pr \left[ \given{I_{k+1}^x-I_{k'+1}^y \neq r_1}{I_{k}^x-I_{k'}^y=r_1} \right] \leq O(1/\sqrt{d}).
	\]
	Assuming this, the two walks make $U_1$ unsynchronized steps, then $S_1$ synchronized steps with $S_1 \sim \mrm{Geom}(O(1/\sqrt{d}))$ distributed geometrically. The walks then make another $U_2$ unsynchronized steps, with~\cite[Lemma 5]{DKK18} yielding $\be[U_2] \leq O(d^{1/4})$, followed by $S_2$ synchronized steps with $S_2 \sim \mrm{Geom}(O(1/\sqrt{d}))$. The process continues this way until one of the walks has completed its $\sqrt{d'}$ steps. Using Lemma~\ref{lem:geoms}, the expected number of such phases of synchronization-unsychronization is $\leq O(d' \sqrt{1/d} + 1) = O(1)$. Combining this with the fact that $\be[U_k] = O(d^{1/4})$, we deduce that the expected number of unsynchronized $i$-steps is $O(d^{1/4})$. Each such step involves $\sqrt{d'}$ $j$-steps, so the total number of queries with non-shared $i$ is $O(d^{3/4})$.
	
	Regarding the steps with shared $i$ and non-shared $j$, random-walk arguments similar to the above argument imply that since on each shared $i$, the two $j$-walks start with distance $O(\sqrt{d})$, and have steps of size $\Theta(d^{1/4})$, they are expected to meet after $O(d^{1/4})$ queries (follows from~\cite[Lemmas 3,5]{DKK18}). Since there are $O(\sqrt{d})$ $i$-steps, the total number of such non-shared queries is $O(d^{3/4})$ as well.
	
	\medskip\noindent \textbf{\textit{Claim 3)}} Similarly to the previous claim, the queries made by stages before $\textsc{stage3}$ are confined to a square area of size $(d^{3/4}+\sqrt{d})\times (d^{3/4}+\sqrt{d})$, and because the input is shifted by $2d^{3/4}$, the queries of $\textsc{stage3}$ do not overlap previous ones. It is clear that once the two walks of $\textsc{stage3}$ on $x$ and on $y$ are synchronized, they remain synchronized. Let $T$ be the total number of steps until the two walks share a point. There are at most $\min(2T, d')$ steps which are not shared, and the failure probability is $\leq \min(2T, d') / d'$, similarly to the proof of Lemma~\ref{lem:min-hash-pr}. Thus, it is sufficient to verify $\be[\min(T, d)] \leq d^{7/8}$. Clearly, after $|i_1^x-i_1^y|$ steps, the walks are being synchronized with respect to the $i$-axis. Let $J$ denote the random variable measuring their distance on the $j$-axis, once the walks first share this same $i$. Since each of the advances of $j$ are independent of the other steps,
	\[
		\be[J^2] = |j_1^x - j_1^y|^2 + \sum_{t=0}^{|i_1^x-i_1^y|} \be[S_t^2],
	\]
	where $S_t$ is the jump on the $j$-axis on the $t$-step of the runner-up walk. In particular $\be[S_t^2] \leq ((d/3)^{3/8})^2 \leq d^{3/4}$. Since $|i_1^x-i_1^y| \leq 2d^{3/4}$, we overall deduce $\be[J^2] \leq O(d^{3/2})$.
	
	From this point on, the walks of $\textsc{stage3}(x, d')$ and $\textsc{stage3}(y, d')$ keep being aligned with respect to the $i$-axis. Once they meet on the $j$-axis, they will remain synchronized. The distance on the $j$-axis between the walks can be modeled as a one dimensional random walk, starting at $J$, and having independent steps whose lengths are a difference of two independent uniform $U(0, 2d'^{3/8})$ variables. Once this difference walk hits $0$, the walks keep being synchronized. Lemma~\ref{lem:sparse_walks} then immediately yields
	\[
		\be[\min(T, d')] \leq |i_1^x-i_1^y| + O\left( (d'^{3/8}+\be[J]/d'^{3/8})\sqrt{d'} \right).
	\]
	Substituting $\be[J]^2 \leq \be[J^2] = O(d^{3/2})$, we obtain $\be[\min(T, d')] \leq d^{7/8}$, as required.
\end{proof}


%\ynote{Let's conclude this section with a formal statement and proof of Theorem~\ref{thm:2dupper} (or whatever we end up feeling comfortable with including). }

\subsubsection{Conjectured optimal algorithm}\label{app:2Dopt}
The 2D-LPHS algorithms presented in the previous sections have the property of not treating both axes symmetrically. For example, $\textsc{Recursive-Hash}$ iterates over several $i_{0}$'s, and for each of them it makes many queries of the form $x[i_0, j]$ for different $j$'s. Except for not being aesthetic, this asymmetry has other disadvantages. For example, it is not obvious how to generalize these algorithms to higher dimensions. More importantly, these algorithms (that we considered) do not have optimal dependence of $\delta$ on $d$.

We conjecture that the following symmetric algorithm (\textsc{Random-Walk-Hash}) has the optimal performance of $\delta = \widetilde{O}(1/d)$. However, we were not able to rigorously analyze it.

%The algorithm together with a heuristic analysis appear in appendix~\ref{app:2Dopt}

\begin{algorithm}
Let $\psi_{1}, \psi_{2}\colon \Sigma_b \to \{-L, \ldots, L\}$ be independent random functions \\
	\Begin{
		$P \gets \mathrm{list}()$ \\
		\For{$s \gets 0\ldots d-1$}{
			$P[s] \gets (i,j)$\\
			$v \gets z[i,j]$\\
			$(i,j) \gets (i + \psi_{1}(v), j + \psi_{2}(v))$\\
			\If{$(i,j) \in P$} {
				Let $t$ be the only index satisfying $P[t]=(i,j)$\\
				$k \gets \mathrm{arg\,min}_{u\in [t,s]} \{z[P[u]]\}$\\
				$(i,j)\gets P[k]$\\
				\While{$(i,j) \in P$} {
					$j \gets j+1$
				}
			}
		}
		\Return $\mathrm{arg\,min}_{(i',j')\in P} \{z[i',j']\}$
	}
	\caption{\textsc{rw-stage}$(z \in \Sigma_b ^{\integers_n^2}, d \in \pintegers, L \in \pintegers, i \in \integers_{n}, j \in \integers_{n})$}
\end{algorithm}
\begin{algorithm}\label{alg:2Doptimal}
	\Begin{
		$I \gets \lg \lg (d)$\\
		$d' \gets d / I$\\
		$(i_0, j_0) \gets \textsc{Min-Hash}(z,\ d')$\\
		$(i_1, j_1) \gets \textsc{rw-stage}(z,\ d',\ d'^{1/4},\ i_0,\ j_0)$\\
		$(i_2, j_2) \gets \textsc{rw-stage}(z,\ d',\ d'^{3/8},\ i_1,\ j_1)$\\
		$(i_3, j_3) \gets \textsc{rw-stage}(z,\ d',\ d'^{7/16},\ i_2,\ j_2)$\\
		$\vdots \qquad \vdots\qquad \vdots\qquad \vdots\qquad \vdots\qquad \vdots\qquad \vdots\qquad \vdots\qquad \vdots$\\
		$(i_I, j_I) \gets \textsc{rw-stage}(z,\ d',\ \sqrt{d'/2},\ i_{I-1},\ j_{I-1})$\\
		\Return $(i_I, j_I)$
	}
	\caption{\textsc{Random-Walk-Hash}$(z \in \Sigma_b ^{\integers_n^2},d \in \pintegers)$}
\end{algorithm}

\paragraph{Heuristic performance}
Here we heuristically describe why we expect the algorithm \textsc{Random-Walk-Hash} to achieve $\delta = \widetilde{O}(1/n)$. %\ohad{Explain the connection to Gaudry-Schost algorithm?}

The main heuristic assumption we make is that each $\textsc{rw-stage}(x, d, L, i, j)$ can be modeled by a random walk on $\integers^{2}$, starting at $(i,j)$ and having independent steps which are uniformly distributed on each axis as $\sim U(-L, L)$. We further assume that once the two walks of $\textsc{rw-stage}(x)$ and $\textsc{rw-stage}(y)$ are synchronized (collided), they remain synchronized. Moreover, we recall that the output location of a $\textsc{rw-stage}(x)$ is the point visited in this walk having the minimal $x$-value.\footnote{These assumptions are not precise mainly because we need the steps to be both determinstic and independent (with respect to the input's randomness) of the previous steps. In practice we cannot guarantee independence, which makes us run into loops. We try to break these in a canonical way. This complicates the analysis.}

Once these assumptions are made, an analysis of \textsc{Random-Walk-Hash} would follow from the following two claims:
\begin{itemize}
	\item Let $T$ be (a random variable measuring) the time that two random walks on $\integers^{2}$, starting at distance $D$ (in $L_{1}$ norm), and making steps distributed as $U(-L, L)$, meet. Then $\be[\min(d',T)] \leq O(\sqrt{d'}(L + D/L))$.
	We say that walks $A,B$ `meet' in time $t$ if $t$ is minimal so that $\exists i,j \leq t$ with $\mathrm{location}_{i}(A)=\mathrm{location}_{j}(B)$.
	\item The expected distance (in $L_{1}$) of a 2D-walk with $d'$ steps distributed as $U(-L, L)$, between the starting point and the final one, is $O(L\cdot \sqrt{d})$
\end{itemize}
Let us analyze the first few stages of \textsc{Random-Walk-Hash} using these claims (which we do not prove here).

Just after the first stage, which is \textsc{Min-Hash}, the walks of $\textsc{Random-Walk-Hash}(x)$ and 
$\textsc{Random-}$ $\textsc{Walk-Hash}(y)$ are synchronized except for probability $O(1/\sqrt{d'})$ (Lemma~\ref{lem:min-hash-pr}), and in case of this failure event, the distance of the two walks has expected value $O(\sqrt{d'})$.

At the second stage, $\textsc{rw-stage}(x,d',d'^{1/4})$, the initial distance between the walks is $D=O(d'^{1/2})$ and $L=d'^{1/4}$. Using the above claims, and a Markov inequality, the random walks would synchronize except for probability $O(D/L+L)\sqrt{d'}/d' = O(d'^{-1/4})$, and in case of failure, the expected distance is $O(d'^{3/4})$.

At the third stage, $\textsc{rw-stage}(x,d',d'^{3/8})$, $D = O(d'^{3/4}), L=d'^{3/8}$ and the failure probability becomes $O(d'^{3/8})/\sqrt{d'}=O(d'^{-1/8})$, and the distance upon failure is $=O(d'^{7/8})$.

Continuing this heuristic to later stages we get that the total failure probability, which is the product of failure probabilities of all the stages, is $2^{O(I)}/d'=\widetilde{O}(d^{-1})$.


\subsection{Lower bounds on 2D-LPHS algorithms}
\label{sec:sub:lower}

%\ynote{Here too, it is better to use the terminology and notation for LPHS from the definitions section.}

In this section we prove Theorem~\ref{thm:kdlower} for $k=2$ (i.e., 2D-LPHS). The proof for any other value of $k > 1 $ is similar. In particular, we show that any 2D-LPHS algorithm satisfies $\delta \geq \Omega(1/d)$, given $n \geq 2d$. (On the other hand, we expect that for cyclic LPHS in the regime of $n = o(d)$, $\delta = o(1/d)$ is achievable, as in Lemma~\ref{lem:crandomw} for one dimension.) The proof of the following auxiliary lemma appears in Appendix~\ref{app:2DLB}.

\begin{lemma}[Bigger shifts]\label{lem:2Dextension}
	Let $h$ be a 2D $(n,b,d,\delta)$-LPHS. Let $r_{1}', r_{2}' \in \pintegers$, and $y'=x' \ll (r_1', r_2')$ where $x' \in \Sigma_b^{\integers_{n}^2}$ is a uniformly random string. Then,
	\[
	\pr\lbs h(x', d) - h(y', d) \rbs \leq \max\{r_1', r_2'\}\delta.
	\]
\end{lemma}
The following lemma implies Theorem~\ref{thm:kdlower} for $k=2$.
\begin{lemma}\label{lem:2DLB}
For $n > 2d$ and any $b > 0$, every 2D (cyclic or non-cyclic) $(n,b,d,\delta)$-LPHS satisfies $\delta \geq 1/(3d)$.
\end{lemma}

\begin{proof}
	Consider the set of queries $P$ made to a uniformly random string $x \in \Sigma_b^{\integers_{n}^2}$ by $A(x, d)$. That is, $P$ is a random variable whose values are sets of sizes $\leq d$ of $(i,j)$ pairs.
	
	Let $x', y' \in \Sigma_b^{\integers_n^2}$ be two uniformly random strings related by $y' = x' \ll (r_1', r_2')$ for uniform independent variables $r_1', r_2' \sim U(0, 2d)$.	
	Using Lemma~\ref{lem:2Dextension},
	\begin{equation}
	\begin{split}
	\pr[h(x',d)-h(y',d) \neq (r_1', r_2')] & = \be_{r_1', r_2'} \lbs \be\lbs \given{h(y',d)-h(x',d) \neq (r_1', r_2')}{r_{1}', r_{2}'} \rbs \rbs \\
	& \leq \be_{r_{1}', r_{2}'} \lbs \max(r_{1}', r_{2}')\delta \rbs \leq 2d\delta.
	\end{split}
	\end{equation}
	
	Let $P_{x'}, P_{y'}$ be copies of $P$ which are the set of queries issued by $h(x', d), h(y', d)$, respectively. Generally, the random variables $P_{x'}, P_{y'}$ are dependent. However, we are going to see they are only slightly dependent. Indeed, suppose $P_{1}, P_{2}$ are two values of $P$. We claim that given specific values of $r_{1}', r_{2}'$ (call these $r_1'', r_2''$) so that $P_{1}$ and (the Minkowski sum) $P_{2} + \{(r_1'', r_2'')\}$ are disjoint, we have
	\begin{equation}\label{eq:lbdis}
	\pr\lbs \given{P_{x'} = P_{1} \wedge P_{y'} = P_{2}}{(r_{1}',r_{2}')=(r_{1}'', r_{2}'')} \rbs = \pr\lbs P = P_{1}\rbs \cdot \pr\lbs P = P_{2}\rbs.
	\end{equation}
	This is because the event $P_{x'} = P_{1}$ is in the $\sigma$-algebra generated by the random variable $\restrict{x'}{P_{1}}$ (that is, events depending only on $\restrict{x'}{P_{1}}$)\footnote{If the LPHS is probabilistic, then we should add the algorithm's randomness into the $\sigma$-algebra. Since this randomness is independent of all other random variables, it doesn't change the proof.}, which is independent of the $\sigma$-algebra generated by $\restrict{y'}{P_{2}}$ (or $\restrict{x'}{P_{2} + \{(r_1'', r_2'')\}}$), as different entries of $x'$ are independent.
	Consider the conditional random variable
	\[
		X_{r_{1}'', r_{2}'', P_{1}, P_{2}} \ddd \lbs \given{h(x',d)-h(y',d)}{r_1'=r_1'', r_2'=r_2'', P_{x'}=P_1,P_{y'}=P_2} \rbs,
	\]
	and compute
	\begin{equation*}
	\begin{split}
	\pr[h(x',d)&-h(y',d) = (r_1', r_2')]\\
	&= \be_{r_1', r_2', P_{x'}, P_{y'}} \lbs \pr\lbs \given{h(x',d)-h(y',d) = (r_1', r_2')}{r_1', r_2',P_{x'}, P_{y'}} \rbs \rbs \\
	&= \be_{r_1', r_2'} \lbs \sum_{P_1, P_2} \pr\lbs X_{r_1',r_2',P_1,P_2} = (r_1',r_2')\rbs \cdot \pr\lbs \given{P_{x'}=P_1,P_{y'}=P_2}{r_1', r_2'}\rbs \rbs \\
	& \stackrel{(a)}{\leq}
	\underbrace{\be_{r_1', r_2'} \lbs \sum_{\substack{P_1, P_2 \colon\\ ((r_1', r_2') \in P_{1} - P_{2})}} \pr\lbs \given{P_{x'}=P_1,P_{y'}=P_2}{r_1', r_2'}\rbs \rbs}_{Q_{1}} + \\
	&+\underbrace{\be_{r_1', r_2'} \lbs \sum_{\substack{P_1, P_2 \colon\\ ((r_1', r_2') \notin P_{1} - P_{2})}} \pr\lbs X_{r_1',r_2',P_1,P_2} = (r_1',r_2')\rbs \cdot \pr [P=P_1] \pr[P=P_2] \rbs}_{Q_{2}} \\
	& \stackrel{(b)}{\leq} \frac{d^{2}}{(2d+1)^2} + \frac{1}{(2d+1)^2} = \frac{d^2+1}{(2d+1)^2}
	,
	\end{split}
	\end{equation*}
	where $P_{1} - P_{2}$ is a Minkowski difference.
	Inequality $(a)$ follows from~\eqref{eq:lbdis} and the fact that probabilities are upper bounded by $1$. Inequality $(b)$ is the key argument. To bound $Q_{1}$ (by $d^2/(2d+1)^2$) we use
	\[
	Q_{1} + \underbrace{\be_{r_1', r_2'} \lbs \sum_{\substack{P_1, P_2 \colon\\ ((r_1', r_2') \notin P_{1} - P_{2})}} \pr [P=P_1] \pr[P=P_2] \rbs}_{Q_{3}} = 1.
	\]
	Exchanging summation order and using $\lba P_{1} - P_{2} \rba \leq |P_{1}|\cdot |P_{2}| \leq d^2$, which holds since $A(x,d)$ makes at most $d$ queries, we see that $Q_{3} \geq 1-d^2/(2d+1)^2$. Notice we use here $n > 2d$. This proves $Q_{1} \leq d^2 / (2d+1)^2$.
	
	To bound $Q_{2}$, we note that every $(P_1, P_2)$ contribute at most
	\[
	\pr[P=P_1]\pr[P=P_2]/(2d+1)^2
	\]
	to $Q_{2}$. To see this, observe that the distribution of the random variable $X_{r_1'',r_2'',P_1,P_2}$ does not depend on the particular value of $r_1'', r_2''$ (given $P_1 + (r_1'', r_2'')$ is disjoint from $P_2$),
	and it attains at most one value (that is, a random variable $X$ and a set $E$ always satisfy $\sum_{e \in E} \pr[X=e]\leq 1$).
	Hence
	\[
	Q_{2} \leq \sum_{P_1, P_2} \frac{\pr[P = P_1] \pr[P = P_2]}{(2d+1)^2} = \frac{1}{(2d+1)^2}.
	\]
	
	Overall, we deduce $2d\delta + (d^2+1)/(2d+1)^2 \geq 1$, implying $\delta \geq 3/(8d)$.
\end{proof}

\begin{remark}
	The proof of Lemma~\ref{lem:2DLB} readily extends to a lower bound on the error probability of any LPHS of higher dimensions. That is, for an LPHS of dimension $k$ one achieves $\delta \geq 1/(3d^{2/k})$ whenever $n>(2d)^{2/k}$, implying Theorem~\ref{thm:kdlower}.

	The essential outline to a general dimension $k$ is as follows: First, we use a distance-extension lemma, analogous to Lemma~\ref{lem:2Dextension}, in a way similar to~\eqref{eq:aaa}. This step reduces our task to showing that no algorithm can synchronize on random inputs $x,y \in \Sigma_b^{\integers_n^k}$ with probability higher than, say $1/2$, where $y$ is a random $k$-dimensional shift of $x$ by about $(2 d)^{2/k}$ in every axis.

	Then, we observe that in the event that the LPHS applied on $x$ and $y$ queries disjoint input cells (we think of $x$ and $y$ as inlaid in a common landscape), synchronization is unlikely, as expressed by the bound on $Q_2$ in the proof of Lemma~\ref{lem:2DLB}. Hence, the synchronization probability is dominated by the probability that the LPHS queries a shared input cell. To bound this latter probability we use a birthday-paradox argument similar to the bound on $Q_1$ in the proof of Lemma~\ref{lem:2DLB}: there are at least $((2d)^{2/k})^k = 4d^2$ possible shifts, while there are only $d \times d$ pairs of queries that may collide -- any of the $d$ queries made to $x$ may collide with any of the $d$ queries made to $y$. We conclude that there is a probability of at most $1/4$ to have a shared query, concluding the argument.
\end{remark}


==> Introduction-Elette.tex <==
%!TEX root = ../LPHS-ICALP.tex

\section{Introduction}

A {\em locality-preserving hash function}~\cite{LinialS96,IndykMRV97}  is a distance-respecting mapping from a complex input space to a simpler output space.
Inspired by recent results in cryptography, we study a new kind of locality-preserving hash functions that map strings to integers while respecting the {\em shift} distance
%\footnote{In this work, the term ``shift distance'' refers to the minimal shift amount required to obtain one string from the other. In the non-cyclic case this corresponds to directed distance in the De Bruijn graph, whereas in the cyclic case the distance is infinite if there is no such shift. Our notion of shift distance should not be confused with an alternative notion (cf.~\cite{andoni2013homomorphic}) referring to the smallest Hamming distance between one string and some cyclic shift of the other. }
between pairs of input strings with high probability. A distinctive feature of these hash functions is that they can be computed in {\em sublinear time} while maintaining low error probability.
%This makes them a useful tool for ``sensing'' relative locations in an unknown environment by taking sublinear-size samples of the surroundings.

\paragraph{\bf Why shifts? Why sublinear?}
Our hash functions for shifts can be thought of as {\em sublinear-time location sensors} that measure a relative position in an unfamiliar environment by taking a sublinear-size sample of the surroundings. This can apply in a variety of settings. For instance, ``surroundings'' may refer to a local view of an unexplored territory, a long string such as a DNA sequence, an external signal such as a GPS synchronization sequence, a digital document such as big pdf file or a virtual world, or a huge mathematical object such as a cryptographic group. See~\cite{AndoniIKH13,ohlsson2014compressive}  for applications of shift finding to GPS synchronization, image alignment,  motion estimation, and more.
%While in some of the above examples local views tend to be noisy, in others they are not. For instance, a local view of a digital document or a mathematical object is noiseless. Finally,
We will discuss additional cryptographic and algorithmic applications in Section~\ref{sec-introapps} below.
We are motivated by scenarios in which the local view contains an enormous amount of relevant information that cannot be naively sub-sampled or compressed. This calls for {\em sublinear-time} solutions.  
Shift finding is quite unique in that it gives rise to nontrivial sublinear-time computable hash functions that do not exist for related metrics. For instance, such hash functions provably do not exist if we replace sequence similarity by set similarity (see Appendix~\ref{app:setsim}).


\paragraph{\bf Simple shift-finding solutions.} To motivate the new primitive,
% in the context of shift-finding problems,
consider the following simple shift-finding problem. An $n$-bit string $x$ is picked uniformly at random, and then cyclically shifted by $s$ bits the left, for some $0\le s < n$. Let $y$ be the resulting string. For instance, $x,y$ may be obtained by measuring the same periodic signal at different phases. We write $y=x\ll s$. The
%(noiseless)
shift-finding problem is to find the shift amount $s$ given $x$ and $y$. %(Note that, except with $2^{-\Omega(n)}$ probability, $s$ is uniquely defined.)
%Different variants of this problem are motivated by applications such as GPS synchronization, image alignment,  motion estimation, and more; see~\cite{AndoniIKH13,ohlsson2014compressive} and references therein. We will discuss additional applications in Section~\ref{sec-introapps} below.
%The shift-finding problem can also be seen as a toy version of the more complex and better studied problem of computing edit distance.
%, and can be useful for other string matching problems.
%See Section~\ref{sec-related} for related work.

In a centralized setting, where $x$ and $y$ are both given as inputs, it is easy to solve the problem  in sublinear time (with small error probability), querying only $\tilde O(n^{1/2})$ bits of the input, by matching substrings of $x$ of length $\ell=O(\log n)$ starting at positions $1,2,\ldots, \sqrt{n}$ with length-$\ell$ substrings of $y$ whose starting position is a multiple of $\sqrt{n}$. (This is a simplified version of a noise-resilient algorithm from~\cite{AndoniIKH13}.) This algorithm is nearly optimal, since any shift-finding algorithm
for an unbounded shift amount $s$
should read $\Omega(\sqrt{n})$ bits of the input~\cite{BatuEKMRRS03}.

In a distributed setting, a natural goal is to design a {\em sketching} algorithm that compresses a single input into a short sketch, such that given the sketches of $x$ and $y$ one can recover $s$ with high probability. Note that the previous centralized algorithm does imply such a sublinear-size sketch, but only with $\tilde O(\sqrt{n})$ output size, which is far from being optimal. Instead, one could use the following classical approach~\cite{Cover}:
%(see~\cite{Cover}, page 144):
let the sketch of $x$ be an integer $0\le z_x<n$ that minimizes $x\ll z_x$ (viewed as an $n$-bit integer), and similarly for $y$. It can be easily seen that $s=z_x-z_y \mod n$ whenever the minimum is uniquely defined. The logarithmic sketch size of this solution is clearly optimal. Moreover, this solution achieves something even stronger than sketching: it yields a hash function $h:\{0,1\}^n\to\integers_n$ that respects cyclic shifts in the sense that for a random input $x$,  we have $h(x)=h(x\ll s)+s$ except with small probability. That is, shifting the input by $s$ changes the output by $s$ in the same direction. This feature can be useful for many applications. For instance, given $t$ hashes $z_i=h(y_i)$, where $y_i=x\ll s_i$ for $i=1,\ldots,t$, one can easily compute in time $\tilde O(t)$ the correct sequencing of the $y_i$. It can also be easily used to obtain a {\em locality-sensitive hash function} (LSH) for cyclic shifts, which maps ``close'' strings to the same output with high probability and ``far'' strings to the same output with lower probability. LSH have applications to nearest-neighbor data structures and  more~\cite{IndykM98,KushilevitzOR98,GionisIM99,APR18,AlucOD19}.

The main downside of the above hashing-based solution compared to the centralized algorithm is its linear running time. A natural question is whether one can obtain the best of both worlds:
\begin{quote}
{\em Can we combine the sublinear running time of the centralized algorithm with the optimal sketch size and locality-sensing features of the hashing-based solution?}
\end{quote}

\subsection{Our Contribution}

%Motivated by the above question and its applications, we
We initiate a  study of hashing-based solutions to the shift-finding problem. We capture such solutions via the following notion of locality-preserving hash function for shifts.

\begin{definition}%[LPHS]
A function $h:\{0,1\}^n\to \integers_n$ is a $(d,\delta)$ {\em locality-preserving hash function for shifts} (LPHS) if: (1) $h$ can be computed by (adaptively) querying $d$ bits of its input, and (2) $\pr \lbs h(x) \neq h(x \ll 1) + 1 \rbs \leq \delta$, where $x$ is random and $\ll 1$ denotes a cyclic shift by one bit to the left.
\end{definition}
Note that, by a union bound, an LPHS as above satisfies $\pr \lbs h(x) \neq h(x \ll s) + s \rbs \leq s\cdot \delta$ for any shift amount $0\le s<n$. Thus, an LPHS has a better accuracy guarantee for smaller shifts. Intuitively, an LPHS can be thought of as a sublinear-time computable location identifier that suffices (with high probability) for determining the exact relative location with respect to adjacent identifiers.
%This will be useful for a variety of applications we discuss below.

%low-resolution snapshot of one's immediate surroundings that suffices (with high probability) for identifying the exact relative location with respect to adjacent snapshots.

\paragraph{Other LPHS flavors.} The above notion of LPHS addresses the basic shift-finding problem as discussed above, but is limited in several important ways: it only considers cyclic shifts and 1-dimensional inputs,
%it is not noise-resilient,
and it only guarantees average-case correctness for uniformly random inputs. To address these limitations, we additionally consider other flavors of the basic LPHS notion defined above that are more suitable for applications. These include a  {\em non-cyclic} variant, where instead of $x\ll 1$ we remove the leftmost bit of $x$ and add a random bit on the right; a {\em $k$-dimensional} variant, where the input is a $k$-dimensional matrix and the output is in $\integers_n^k$;
%a {\em noise-resilient} variant, where each bit of the shifted input is flipped with probability $\epsilon$;
and a {\em worst-case} variant where the quantification is over an arbitrary $x$ that is ``far from periodic'' and the probability is over the choice of $h$. Most of the new applications we present require at least one of these extensions.

\subsubsection {Near-Optimal LPHS via Distributed Discrete Log}

We establish a general two-way connection between LPHS and algorithms for the {\em distributed discrete logarithm} (DDL) problem~\cite{BGI16}. Before explaining this connection, we start with relevant background.

The traditional discrete logarithm (DL) problem is parameterized by a cyclic group $\mathbb G$ of order $n$ with a generator $g$, where $n$ is typically a large prime. The challenge is to recover a random $u\in\integers_n$ from $g^u$. Many cryptographic applications
%, including widely deployed ones,
rely on the conjectured intractability of the DL problem in special types of groups, including subgroups of $\integers^*_p$ and certain families of elliptic curves.
%However, all such constructions can be broken in quantum polynomial time via Shor's algorithm.

The DDL problem is a distributed variant of the DL problem that was recently introduced in the context of group-based homomorphic secret sharing~\cite{BGI16}. In DDL there are two parties, where the first party's input is $g^u$ for a random $u$, and the second party's input is $g^{u+s}$ where $s\in\{0,1\}$ (more generally, $s$ can be a small integer). The goal is for each party to locally output an integer, such that the difference between the two outputs is $s$. One can assume without loss of generality that the two parties run the same algorithm.

Note that a DL algorithm can be used to perfectly solve the DDL problem. However, this is computationally infeasible in a cryptographically hard group, where $n$ is enormous. Instead, a DDL algorithm uses a bounded running time (typically polylogarithmic in the group order $n$) to obtain the correct difference except with error probability $\delta$. For instance,
%the solution \emph{MinHash}
%Yuval: the MinHash solution is actually different
the initial solution proposed in~\cite{BGI16} uses a pseudorandom function to mark each group element as ``distinguished'' with probability $\delta$, and makes each party, on input $v$, output the smallest $z\ge 0$ such that $v\cdot g^z$ is distinguished. The (expected) running time of this algorithm is roughly $1/\delta$, and the error probability is $\delta$ (corresponding to the case where $s=1$ and $g^u$ is distinguished).

The DDL problem can be related to the LPHS problem (over a non-binary alphabet) by associating each party's DDL input $v$ with an LPHS input consisting of the sequence of group elements $x=(v,  gv, g^2v,\ldots, g^{n-1}v)$. Indeed, multiplication of the DDL input by $g$ corresponds to a cyclic shift of $x$ by one symbol to the left. We formalize this intuition by proving a general two-way relation between LPHS and DDL algorithms in the {\em generic group model}~\cite{S97}, where group elements are assigned random labels and the algorithm is only given oracle access to the group operation.

The applications we derive from the above connection give an unusual example for the usefulness of results on group-based cryptography in a post-quantum world. Indeed, all traditional applications of group-based cryptography are subject to quantum polynomial-time attacks using Shor's algorithm, and are thus useless in a post-quantum world. If scalable quantum computers become a reality, cryptosystems that are ``quantum broken'' will become obsolete. In contrast, sublinear-time classical algorithms will still be meaningful even in a post-quantum world.
%, regardless of the speedup that can be achieved by a quantum computer. This is due to a quantifier difference between cryptography and algorithms: whereas cryptography considers security against worst-case attackers, algorithms optimize for honest parties.

\paragraph{\bf LPHS constructions.} The simple DDL algorithm from~\cite{BGI16} corresponds to a $(d,\delta)$-LPHS where $\delta=\tilde O(1/d)$. Another simple LPHS construction with similar parameters, implicit in a DDL algorithm from~\cite{BGI17}, makes a simple use of MinHash~\cite{BroderCFM00}: let $h(x)$ output the index $i$, $1\le i \le d$, that minimizes the value of a MinHash applied to a polylogarithmic-length substring of $x$ starting from $x_i$.

It is tempting to conjecture that the above simple LPHS constructions are near-optimal, in the sense that $\delta=o(1/d)$ is impossible. It turns out, however, that a quadratic improvement can be obtained from a recent optimal DDL algorithm due to Dinur et al.~\cite{DKK18}. This \emph{Iterated Random Walk (IRW)} algorithm, whose self-contained description appears in Appendix~\ref{sec:dkk}, is based on a carefully chosen sequence of random walks in the group. It can be viewed as a non-trivial extension of Pollard's classical ``kangaroo'' DL algorithm~\cite{Pollard78}, which runs in time $\tilde O(\sqrt{n})$ and has low space complexity. Applying the LPHS vs.\ DDL connection to the DDL results from~\cite{DKK18}, we get the following theorem.

\begin{theorem} [Near-optimal LPHS]\label{th-main}
There exist $(d,\delta)$-LPHS with: (1) $\delta= \tilde{O}(d^{-2})$ for $d\le\sqrt{n}$,
and (2) $\delta = n^{-\omega(1)}$ for $d = \tilde{O}(\sqrt{n})$. Furthermore, both ``$\delta= \tilde{O}(d^{-2})$'' in (1) and ``$d = \tilde{O}(n^{1/2})$'' in (2) are optimal up to polylogarithmic factors.
\end{theorem}

Interestingly, any sublinear-time LPHS must inherently make adaptive queries to its input.
%In fact, we prove (Section~\ref{sec-sketching}) that adaptive queries are necessary even in the relaxed setting of sketching.
Adaptive queries are unusual in the context of sublinear metric algorithms, but were previously used in sublinear algorithms for approximating and embedding edit distance~\cite{Saha14,ChakrabortyGK16,GoldenbergKS19,KociumakaS20}.


\paragraph{\bf Additional variants.} We prove similar bounds for the worst-case and non-cyclic variants of LPHS. The result for the worst-case variant is obtained via a general reduction, and inevitably excludes a small set of inputs that are close to being periodic. The result for the non-cyclic case does not follow generically from the cyclic case (except when $d<n^{1/3}$), and requires a special analysis of the IRW algorithm~\cite{DKK18}. Also, in this case only  (1) holds, since the error probability of a non-cyclic LPHS must satisfy $\delta=\Omega(1/n)$ regardless of $d$. In fact, whereas $d = \sqrt{n}$ is the hardest case for Theorem~\ref{th-main} in the non-cyclic case (in that (1) for $d = \sqrt{n}$ easily implies (1) for smaller $d$), it is the easiest for the cyclic case (in that it is implied by the simpler algorithm of Pollard~\cite{Pollard78}).
%Finally, one can use recent results on DL with preprocessing~\cite{Corrigan-GibbsK18} to show that, in the cyclic case, bounded-length shift-invariant advice on $x$ cannot improve the parameters by much.

In the context of {\em sketching} for shifts, the above results imply solutions that simultaneously achieve near-optimal sketch size of at most polylog$(n)$, near-optimal running time of $\tilde O(\sqrt{n})$, and negligible error probability, for both cyclic and non-cyclic shifts, and for arbitrary ``far-from-periodic'' inputs.
\iffalse
Moreover, assuming a bound $S$ on the shift size $s$ and settling for error probability $\delta=\tilde O(S/n)$, the sketch size can be  reduced to $O(\log S)$. Finally, when $S\le \sqrt{n}$ we can further make this scheme {\em Las Vegas} in the sense that each sketch can output a special symbol $\bot$ with $\le\delta$ probability, and in the event that neither outputs $\bot$ the output must be correct. For instance, with $S=\mathrm{polylog}(n)$ we get a sketch of size $O(\log\log n)$ with $\delta=\tilde O(1/n)$ (Las Vegas) error and $\tilde O(\sqrt{n})$ running time.
\fi

\begin{comment}
\subsubsection{Noise-Resilient LPHS}

The above LPHS constructions assume a noise-free setting. While this suffices for applications that involve digital objects, it may not be realistic for analog data. Here we consider the simple (and standard) case of {\em random} noise, which makes our negative results stronger.
Our positive results can be extended to alternative natural noise distributions, such as bursty noise which is concentrated in blocks of consecutive bits. The case of general adversarial noise (with random $h$) remains open.
% such as noisy GPS signals, different pictures of the same object, or DNA sequences. It is therefore natural to ask if LPHS can be made {\em noise-resilient}. We say that an LPHS is $\eps$-resilient if its error bound $\delta$ holds when each bit in the shifted input is independently flipped with probability $\eps$.

In the context of (centralized) sublinear shift-finding algorithms, non-trivial $\eps$-resilient algorithms were presented in~\cite{AndoniIKH13}.  It turns out that in the more restrictive context of LPHS, only a much smaller amount of noise can be tolerated. We start by stating our positive results.
\begin{theorem}
For
$n = \tilde{\Omega}(d^2)$,
$d<\sqrt{n}$,
there is an $\eps$-resilient $(d,\delta)$-LPHS $h:\{0,1\}^n\to\integers_n$ where
\[
    \delta =
\begin{dcases}
    \tilde{O}(1/d^2),& \eps \leq d^{-3}\\
    \tilde{O}(\eps),         & \eps \geq d^{-1}\\
	\tilde{O}(\sqrt{\eps/d}), &  d^{-3} \leq \eps \leq d^{-1}.\\
\end{dcases}
\]
\end{theorem}

%In the range $\eps \geq d^{-1}$ and $\eps \leq d^{-3}$, we prove that the above upper bounds are tight up to polylogarithmic factors. For the remaining case of $d^{-3} \leq \eps \leq d^{-1}$, there is some gap between our upper and lower bounds. Interestingly, in this case we show that our upper bound is tight (up to polylogarithmic factors) based on a close variant of a seemingly unrelated conjecture of Schramm and Steif~\cite{SS10} on the noise sensitivity of certain Boolean functions.

The upper bound in the range $d^{-3} \leq \eps \leq d^{-1}$ is obtained by an algorithm which combines the algorithms of~\cite{BGI16} and~\cite{DKK18} for the DDL problem. On the negative side, in the range $\eps \geq d^{-1}$ and $\eps \leq d^{-3}$, we prove that the above upper bounds are tight up to polylogarithmic factors. For the more complex case of $d^{-3} \leq \eps \leq d^{-1}$, we obtain the following lower bound:
\begin{theorem}
\label{thm:1dlower_intro}
For $n = \Omega(d^2)$, any (cyclic or non-cyclic) $(n,1,d,\eps,\delta)$-LPHS satisfies
$\delta \geq \eps^{2/3}/d^{1/3}$.
\end{theorem}
We prove Theorem~\ref{thm:1dlower_intro} by reducing it to a seemingly unrelated problem on noise sensitivity of certain Boolean functions, and using a theorem of Schramm and Steif~\cite{SS10} from the field of \emph{percolation theory}.
Interestingly, we show that our upper bound in this case is tight (up to polylogarithmic factors), based on a close variant of a well-known conjecture on noise sensitivity, which Schramm and Steif raised in the same paper.

We similarly obtain nearly tight bounds for noise-resilient LPHS in a more liberal regime, where both the shift bound and the allowed error probability are large. This is a common parameter regime in applications that use LPHS to detect big shifts.


\subsubsection {Multidimensional LPHS}

Viewing LPHS as a location identifier, it is natural to consider a generalization to two dimensions and beyond. Indeed, a 2-dimensional (non-cyclic) LPHS can be useful for aligning or sequencing local views of a big 2-dimensional (digital or physical) object. A $k$-dimensional LPHS maps a $k$-dimensional matrix (with entries indexed by $\integers_n^k$) into a vector in $\integers_n^k$ so that (cyclically) shifting the input matrix by 1 in axis $i$ changes the output vector by the  unit vector $e_i$, except with $\delta$ error probability. As before, this guarantees recovering an arbitrary shift vector with error probability that scales with the $\ell_1$ norm of the shift.

For the 2-dimensional case, we can show the following positive result.
\begin{theorem}
For $d<\sqrt{n}$, there is a 2-dimensional $(d,\delta)$-LPHS with $\delta = \tilde{O}(d^{-7/8})$.
\end{theorem}
The theorem applies also to the non-cyclic case, and is proved via a
%rather complex
specialized algorithm that improves over alternative approaches based on reduction to the 1-dimensional case
whose best error bound is $\delta = O(d^{-4/5})$.

%\medskip \noindent
On the lower bounds side, we prove:
\begin{theorem}
For
%$n>d^2$,
$d<\sqrt{n}$, any $k$-dimensional $(d,\delta)$-LPHS satisfies $\delta = \Omega(d^{-2/k})$.
\end{theorem}
The proof
%is a somewhat complex
of this lower bound is based on an argument involving Minkowski sums and differences of sets in $\mathbb{R}^k$. Finally, for the case $k=2$, we present a heuristic construction that we conjecture to meet this lower bound,  improving over our provable $\delta = \tilde{O}(d^{-7/8})$ bound.

\end{comment}

\subsubsection{Multidimensional LPHS}

Viewing LPHS as a location identifier, it is natural to consider a generalization to two dimensions and beyond. Indeed, a 2-dimensional (non-cyclic) LPHS can be useful for aligning or sequencing local views of a big 2-dimensional (digital or physical) object. A $k$-dimensional LPHS maps a $k$-dimensional matrix (with entries indexed by $\integers_n^k$) into a vector in $\integers_n^k$ so that (cyclically) shifting the input matrix by 1 in axis $i$ changes the output vector by the unit vector $e_i$, except with $\delta$ error probability. As before, this guarantees recovering an arbitrary shift vector with error probability that scales with the $\ell_1$ norm of the shift.

\paragraph{Upper bounds.} In the 2-dimensional case, roughly speaking, the algorithm can be viewed as two parties that are given points $(x,y),(x+\alpha,y+\beta)$ in a random matrix, where $\alpha,\beta \in \{0,1\}$, and their goal is to maximize the probability of synchronizing at the same point, where only $d$ queries are allowed and there is no communication between the parties. A straightforward approach is to use a MinHash algorithm in which the parties take the minimal  hash value computed on values of a $d^{1/2} \times d^{1/2}$ matrix of elements beginning at the location of each party, resulting in a $(d,\delta)$-LPHS with $\delta = \tilde{O}(d^{-1/2})$. A better error bound of $\delta = \tilde{O}(d^{-2/3})$ can be obtained by combining the application of MinHash on one axis with the application of the aforementioned optimal IRW algorithm on the other axis.

We present three improved algorithms in Section~\ref{sec:2dim}. The simplest of those, with a bound of $\delta = \tilde{O}(d^{-4/5})$ is obtained by applying IRW on both axes. This algorithm is described in detail in Section~\ref{sec:2dim}. A natural idea is to first synchronize on the column; then, synchronizing on the row is easy, using the 1-dimensional IRW algorithm. To synchronize on the column, the parties perform the 1-dimensional IRW algorithm with $d/d'$ `horizontal' steps, where the information used to determine each step is distilled from the column in which the current point resides, using an IRW algorithm with $d'$ `vertical' steps. Analysis presented in Section~\ref{sec:2dim} shows that the bound $\delta = \tilde{O}(d^{-4/5})$ is obtained for the parameter $d'=d^{3/5}$.

Our main upper bound is obtained by a more complex algorithm, which -- perhaps, surprisingly -- does not rely on the optimal 1-dimensional IRW algorithm at all. We prove:
\begin{theorem} \label{thm:2dupper}
For $n = \tilde{\Omega}(d^2)$,
%and any $b > 0$,
there is a 2-dimensional
%$(n,b,d,\delta)$-LPHS
$(d,\delta)$-LPHS
with $\delta = \tilde{O}(d^{-7/8})$. There is also a non-cyclic 2-dimensional LPHS with the same parameters.
\end{theorem}
The algorithm we use to prove Theorem~\ref{thm:2dupper} consists of three stages. After each stage the parties either converge to the same location, in which case they stay synchronized to the end of the algorithm, or the two walks are within a bounded distance from  each other. The first stage begins with a distance of at most $1$  on each axis, and is a straightforward application of the 2-dimensional MinHash-based algorithm. The second stage begins with a distance of at most $\sqrt{d}$ on each axis and uses an asymmetric deterministic walk that consists of $\sqrt{d}$ horizontal steps of size $\sim d^{1/4}$, where each step is pseudo-randomly determined by information distilled from a vertical walk of length $\sqrt{d}$ and step sizes $\sim d^{1/4}$. The third stage begins with a distance of at most $d^{3/4}$ on each axis and uses a different deterministic walk. This time, the horizontal steps are of size $1$, while the vertical steps are of size about $d^{3/8}$, and unlike all other steps, can be negative. The analysis of the algorithm relies on martingale techniques.

Finally, we present another 2-dimensional LPHS algorithm, which seems harder to analyze, but for which we conjecture that the error rate is at most $\tilde{O}(d^{-1})$. This bound is near-optimal given the lower bound discussed below. The idea behind this algorithm is to not treat the axes separately but rather to perform a series of deterministic walks over $\mathbb{Z}^2$, with step sizes of about $d^{1/4}, d^{3/8}, d^{7/16},\ldots,\sqrt{d}/2$. Our experiments suggest that the error rate of this algorithm is indeed $\tilde{O}(d^{-1})$. However, the analysis (and especially deterministic resolution of cycles in the random walk) is quite involved and the success probability of this algorithm is left open.

\paragraph{Lower bound.}
%\medskip \noindent
We complement our positive results by proving the following lower bound, extending in a nontrivial way the lower-bound for 1-dimensional LPHS obtained from~\cite{DKK18} via the DDL connection.
\begin{theorem}\label{thm:kdlower}
For
%$n>d^2$,
$2d^{2/k}<\sqrt{n}$, any $k$-dimensional $(d,\delta)$-LPHS satisfies $\delta = \Omega(d^{-2/k})$.
\end{theorem}
The intuition is related to the birthday bound. A $k$-dimensional box with edge length $d^{2/k}$ contains $d^2$ points.
If the $k$-dimensional shift is uniform within this box, we expect the $d$ queries of the two parties not to
intersect with constant probability, implying that $\delta = \Omega(1)$.
Given this, the proof for 
smaller shifts follows by a union bound.
While the intuition is simple, is it not clear how to directly apply the birthday bound, and the formal proof 
is based on an argument involving Minkowski sums and differences of sets in $\mathbb{R}^k$.



%Finally, for the case $k=2$, we present a heuristic construction that we conjecture to meet this lower bound,  improving over our provable $\delta = \tilde{O}(d^{-7/8})$ bound.



\subsubsection{Applications}
\label{sec-introapps}
We present several cryptographic and algorithmic applications that motivate our study of different flavors of LPHS. In particular, all these applications either strongly benefit from or entirely depend on the multidimensional variant of LPHS, and most require the non-cyclic, worst-case variant.

\paragraph{Packed homomorphic secret sharing.}
We demonstrate a cryptographic application of \emph{$k$-dimensional} LPHS in trading computation for communication in group-based homomorphic secret sharing (HSS). In a nutshell, we use LPHS to further improve the succinctness of the most succinct approach for simple ``homomorphic'' computations on secret data, by packing 2 or more plaintexts into a single ciphertext. Compared to competing lattice-based approaches based on homomorphic encryption (see, e.g.,~\cite{AkaviaSWY19} for a recent example), packed HSS provides much better succinctness at a higher computational cost.
The key technical idea is to use a non-cyclic $k$-dimensional LPHS for implementing a $k$-dimensional variant of DDL, where $k$ independent group generators are used for encoding $k$ small integers by a single group element, and where multiplication by each generator is viewed as a (non-cyclic) shift in the corresponding direction. This $k$-dimensional generalization of DDL can be potentially useful for other  recent applications of DDL that are unrelated to HSS~\cite{DottlingGIMMO19,trapdoor2,BrakerskiKM20}.  See Section~\ref{sec-applicationhss} for a detailed discussion of this cryptographic application of LPHS along with the relevant background.

\iffalse
An HSS scheme is a secret sharing procedure which supports compact homomorphic evaluation on secret shares: namely, a method for splitting secret value $s$ into ``shares'' $s_0,s_1$, which individually hide $s$, and which can be locally manipulated as $y_i = \HEval(x_i,f)$, such that the resulting values satisfy $y_0+y_1 = f(s)$. HSS can be viewed as a relaxation of fully homomorphic encryption~\cite{RAD,Gentry09}, with applications including succinct secure computation, private manipulation of remote databases, and more (e.g.,~\cite{GilboaI14,BGI16,WangYGVZ17,BCGIKS19}).
An advantage of HSS over homomorphic encryption is that the output representation is {\em additive}, in the sense that the output is the sum (over a finite group)  and can be easily communicated or used as an input to standard protocols for secure multiparty computation.

Constructions of HSS schemes based on DL-type assumptions (starting from~\cite{BGI16}) were the original motivation of explicitly considering DDL algorithms.  In these schemes, each homomorphic multiplication operation (to multiply $ab \in [M]$ for some maximum plaintext size $M$) resulted in the parties holding group elements $x \in \G$ and $x \cdot g^{a b} \in \G$, where $g$ is a generator of the (cyclic) cryptographically hard group $\G$, and a DDL procedure was used to non-interactively convert these elements to \emph{additive} shares of $ab$ over $\mathbb{Z}_q$ (where $q=|\G|$), with some small but non-negligible error.

Although HSS schemes with better computational efficiency can be achieved from recent developments based on lattices~\cite{EC:BoyKohSch19}, the group-based constructions still remain the optimal choice for \emph{HSS share size} for all but very large secrets.\footnote{While HSS constructions based on Ring Learning with Errors (RLWE) can ultimately provide good \emph{amortized} share size, this requires amortization over thousands of bits of payload, due to the large RLWE-based ciphertext size~\cite{EC:BoyKohSch19}.} Because of this, there is particular motivation for further optimizing the HSS share size of group-based solutions. Indeed, this direction has been explored in~\cite{BCGIO17} as an attractive means for lightweight homomorphic computations on small secrets that may originate from  different clients.

We present a new qualitative optimization, in which a \emph{$k$-dimensional} LPHS (and, in turn, $k$-dimensional DDL) algorithm can be used to obtain a \emph{packed} form of group-based HSS, wherein a single-value HSS share from existing constructions can (roughly) store and operate over a \emph{vector} of $k$ distinct elements. The high-level idea is to use $k$ independent group generators for encoding $k$ integers by a single group element, and view multiplication by each generator as a (non-cyclic) shift in the corresponding direction.

Plugging in our new 2-dimensional LPHS constructions, the resulting approach further reduces the share size of the most succinct known group-based HSS by roughly a factor of 2, while still providing good tradeoffs between homomorphic evaluation time and error probability. We also discuss an alternative approach for packed HSS that uses a non-trivial reduction to 1-dimensional LPHS. While this approach is dominated by our main approach given an {\em optimal} $k$-dimensional LPHS, it can in some parameter regimes provide better time-error tradeoffs than those obtained via our provable constructions of $k$-dimensional LPHS.
\fi
%improvements in the time versus correctness error relation as compared to direct na\"{i}ve embedding approaches.

%\reddit{End of Intro piece}
%\subsection{Related Works}
%\label{sec-related}

\paragraph{Location-sensitive encryption.} We apply LPHS to obtain a sublinear-time solution for {\em location-sensitive encryption} (LSE), allowing one to generate a public ciphertext that can only be decrypted by someone in their (physical or virtual) neighborhood. Here proximity is defined as having significantly overlapping views, and security should be guaranteed as long as a non-overlapping view is sufficiently unpredictable.  The above goal can be reduced to realizing a sublinear-time computable fuzzy extractor~\cite{DORS}\footnote{There are two differences from the  standard notion of fuzzy extractors: the ``distance'' is not a strict metric, and the notion of unpredictability needs to ensure that the source is far from periodic with high probability. }  for shift distance.
Obtaining such fuzzy extractors from LPHS constructions requires an understanding of their behavior on entropic sources. It turns out that even for high-entropy sources, an LPHS provides no unpredictability guarantees. We get around this problem by defining a hash function that combines the output of an LPHS with a local function of the source. Using this approach, we obtain a sublinear-time LSE whose security holds for a broad class of mildly unpredictable sources. See Section~\ref{sec-lse}
% \ynote{placeholder ref}
for the LSE application of LPHS.


\paragraph{Algorithmic applications.} As discussed above, algorithmic applications of LPHS follow from the vast literature on sketching, locality-preserving and locality-sensitive hashing, and metric embeddings. Indeed, our different LPHS flavors can be roughly viewed as probabilistic isometric embeddings of certain shift metrics into a Euclidean space. Thus, for example, an LSH for the same shift metric can potentially follow by concatenating the LPHS with an LSH from the literature. However, some care should be taken in applying this high-level approach. One issue is the average-case nature of LPHS, which makes the failure probability input-dependent. We get around this via a worst-case to average-case reduction that restricts the input space to ``non-pathological'' inputs that are far from periodic. Another issue is that LPHS provides no explicit guarantees for inputs that are too far apart. We get around this by using the fact that an LPHS must have a well-spread output distribution on a random input. As representative examples, we demonstrate how LPHS can be applied in the contexts of communication complexity and LSH-based near-neighbor data structures for shifts.
%For the communication complexity application, we show that the LPHS-based solution is in a sense tight by proving that {\em any} sublinear-time solution should make adaptive queries to the input.  This strengthens a similar result for LPHS implicit in~\cite{DKK18}, replacing a Fourier analytic argument by an information-theoretic argument in the spirit of a recent lower bound from~\cite{HaitnerMORY19}.
The algorithmic applications of LPHS are discussed in Section~\ref{sec-algorithmic}.



%Paper by Robi et al.
\paragraph{\bf Open questions.}
Our work leaves several open questions. While we have a good understanding of the achievable LPHS parameters,
%the noise-resilience of LPHS in the middle range of parameters, resilience to adversarial noise, and
the optimal parameters of $k$-dimensional LPHS (even for $k=2$) are left open.
Another direction concerns the gap between LPHS and the relaxed setting of sketching.
%As discussed above, we show that a
A negative result from~\cite{DKK18}, which can be used to rule out sublinear-time LPHS with non-adaptive queries, in fact holds even for the case of sketching.
%This gives one performance measure for which relaxing locality-preserving hashing to sketching does not help.
Do LPHS-based sketches also provide an optimal tradeoff between sketch size and error probability?

%Another direction is extending LPHS-like solutions to richer classes of metrics. In Appendix~\ref{app:setsim} we rule out a similar sublinear-time computable hash function for a related set similarity metric. What are the distinctive features of metrics supporting sublinear-time locality-preserving hashing?

%Can noise-resilient sketching circumvent our negative results for noise-resilient LPHS?


\paragraph{\bf Organization.}
In Section~\ref{sec:prelims} we introduce necessary preliminaries and notation, including the definition of Locality-Preserving Hash functions for Shifts (LPHS). In Section~\ref{sec:2dim} we present results on multidimensional LPHS, focusing on upper bounds. 
We defer further material to the Appendices. 

%In Appendix~\ref{sec:relations} we formalize the relation between LPHS and generic-group algorithms for the Distributed Discrete Logarithm (DDL) problem and present some useful relations between LPHS variants. A detailed presentation of cryptographic and algorithmic applications of LPHS appears in Appendix~\ref{sec:applications}. Appendix~\ref{??} contains a self-contained summary of results from~\cite{??}. In Appendix~\ref{app:worst-case}  And, in Appendix 



\iffalse
Finally, on the cryptographic applications front, LPHS can provide an attractive means for {\em location-sensitive encryption}, allowing one to efficiently generate a public ciphertext that can only be decrypted by someone in their (physical or virtual) neighborhood.  This goal can be achieved via a fuzzy extractor~\cite{DORS} for a shift metric, assuming that the ``surroundings'' have a sufficient amount of entropy. Obtaining such fuzzy extractors from LPHS requires understanding their behavior on entropic sources, which is left for future work.
\fi

\iffalse
In this work we study a new type of hash function designed for detecting {\em shift amount} between


The problem of detecting the shifts between two strings has recently received
This work connects the problem of detecting shifts in sublinear time
We introduce and study a new type of hash function that embeds

\ynote{ Just rough points for a future intro. }

Algorithmic motivation, locality-preserving / non-expansive hashing, locality-sensitive hashing. Then zoom in on shifts, defining the shift metric (e.g., distance in De Bruijn graph in cyclic case) and mention some broad application domains. Footnote mentioning the alternative shift metric (smallest Hamming distance to a cyclic shift). Explain square-root sublinear-time algorithm (mentioning relevant work) and motivate the stronger notion of hashing.  Distinguish between cyclic and non-cyclic. Discuss average-case vs. worst-case. Discuss inherent limitations of (cyclic and non-cyclic) LPHS:  $\Omega(1/d^2)$ error, and $\Omega(1/n)$ in non-cyclic case.

Present the DDL problem and its relation with cyclic LPHS as our starting point. Say that we can in fact establish a nearly tight two-way connection between DDL algorithms and {\em cyclic} LPHS. Discuss the quantum angle (unusual application of ``group-based crypto'' that is relevant also in a post-quantum world). Explain the problem with a generic derivation of optimal non-cyclic LPHS and why a closer inspection of the DKK analysis does imply it.

\fi


==> Noise-LPHS.tex <==
% !TEX root = ../LPHS.tex


\section{A Lower Bound for the Noisy LPHS Problem}
\label{sec:lower-noisy}


In this section we obtain lower bounds for the noisy LPHS problem, using discrete Fourier analysis and noise sensitivity. Specifically, we prove Theorem~\ref{thm:1dlower}, which asserts the following:

\medskip \noindent \textbf{Theorem~\ref{thm:1dlower}.} For any $(n,1,d,\eps,\delta)$-LPHS, we have
    $$\delta \geq \max(\Omega(1/d^2), \Omega(\eps), \Omega(\eps^{2/3}/d^{1/3})).$$

\medskip \noindent The lower bound $\delta = \Omega(1/d^2)$ holds even for $\eps=0$, i.e., in the non-noisy variant, as was shown in~\cite[Theorem~5]{DKK18}. The lower bound $\delta \geq \Omega(\eps)$ holds even without the shift, i.e., when we consider $\pr_{x \sim_{\eps} y} \lbs h(x) \neq h(y) \rbs$ instead of $\pr_{x \sim_{\eps} y} \lbs h(x) \neq h(y \ll 1) + 1 \rbs$. This follows immediately from~\cite[Lemma~2.2]{MosselO05}, and the following lemma applied with $m = 2$ and $b = 1$ (which implies that $h \bmod 2$ is almost perfectly balanced).
\begin{lemma}\label{lem-smoothness}
Let $m > 1$ be a natural number. Then any $(n,b,d,\delta)$-LPHS satisfies
\[
\Pr_x[h(x) \bmod m = a] \leq m^{-1} + \delta + O(1/n)
\]
for every $a \in \mathbb{Z}_m$.
\end{lemma}
\begin{proof}
We assume that $b = 1$. The proof for $b> 1$ is similar.

Consider the set $S$ of inputs $x$ for which the minimal $r$ such that $x = x \ll r$ is $n$. The set $S$ contains a fraction of $1 - o(1/n)$ of the inputs $x \in \{0,1\}^n$. Suppose first that $m$ divides $n$. Partition the set $S$ into sequences of length $m$ of the form $x,x \ll 1,\ldots,x \ll (m-1)$ and consider the executions $h(x) \bmod m,\ldots,h(x \ll (m-1)) \bmod m$. Note that if $a$ appears $t > 1$ times in an execution sequence, then $h$ must err on at least $t-1$ inputs in this sequence. Consequently,
\[
\Pr_x[h(x) \bmod m = a] \leq m^{-1} + \delta + o(1/n).
\]
If $m$ does not divide $n$, then the set $S$ cannot be accurately partitioned as above.
Consequently, each set of cyclic shifts of any input $x$ (of size $n$) in $S$ may contain at most one additional input $y$ such that $h(y) \bmod m = a$, contributing to the additional $O(1/n)$ factor.
\end{proof}


%\ynote{ Didn't look too carefully, but don't we need to argue first that the output of $h$ on a random input is somewhat uniform? Unless this is really immediate, it may be good to have a short appendix spelling out the details of the $\delta\ge\eps$ proof. }

Next, it remains to prove the following:
\begin{proposition}
\label{prop:lower}
For any $(n,1,d,\eps,\delta)$-LPHS, we have $\delta = \Omega(\eps^{2/3}/d^{1/3})$.
\end{proposition}

We shall prove Proposition~\ref{prop:lower} using a seemingly unrelated theorem of Schramm and Steif~\cite{SS10} regarding the discrete Fourier expansion of certain Boolean functions. We begin with a brief introduction to the discrete Fourier-analytic tools required for the proof, then we proceed with the proof itself, and we conclude with showing that a stronger lower bound of $\Omega(\sqrt{\eps/d})$, which matches the error rate obtained by our algorithm, would follow from a conjecture of Schramm and Steif~\cite{SS10}.

\subsection{Discrete Fourier analysis and noise sensitivity}

For a function $f:\{0,1\}^n \rightarrow \mathbb{R}$, the discrete Fourier expansion of $f$ is its unique representation as a multilinear polynomial over the reals. In other words, it is the expansion $f = \sum_{S \subset [n]} \hat f(S) \chi_S$, where
\[
\chi_S(x) = \prod_{i \in S} (2x_i-1) \qquad \mbox{ and } \qquad \hat f(S) = \frac{1}{2^n} \sum_{x \in \{0,1\}^n} f(x)\chi_S(x).
\]
(The uniqueness of the expansion follows from the set $\{\chi_S\}_{S \subset [n]}$ being an orthonormal basis for the space of real-valued functions on $\{0,1\}^n$.) The coefficients $\hat f(S)$ are called `the Fourier coefficients of $f$'. The \emph{level} of the coefficient $\hat f(S)$ is $|S|$, and the $k$-th level Fourier weight of $f$ is the total weight on $k$-th level coefficients, i.e., $W^k(f)=\sum_{|S|=k} \hat f(S)^2$.

Correlation between functions on the discrete cube has a convenient representation in terms of the Fourier expansion. Indeed, Plancherel's identity implies that for any $f,g:\{0,1\}^n \rightarrow \mathbb{R}$, we have
\[
\be[fg] = \frac{1}{2^n} \sum_{x \in \{0,1\}^n} f(x)g(x) = \sum_{S \subset [n]} \hat f(S) \hat g(S).
\]
As $\hat f(\emptyset) = \be[f]$ for any $f$, it follows that
\begin{equation}\label{Eq:Lower-Aux0}
\cov(f,g) = \sum_{S \neq \emptyset} \hat f(S) \hat g(S), \qquad \var(f) = \cov(f,f) = \sum_{S \neq \emptyset} \wh{f}(S)^{2}.
\end{equation}
A useful tool for analyzing algorithms acting on a distorted input is the \emph{noise operator}. For an $x \in \zo^{n}$ and $\epsilon>0$, $N_{\eps}(x)$ is a random variable distributing over $\zo^{n}$ and having $\forall i\colon \pr[N_{\eps}(x)_i=x_i]=1-\epsilon$ independently of other coordinates. Naturally, the distorted version of a function $f$ is a function $N_{\epsilon}f$ satisfying $\forall x \in \zo^{n}\colon N_{\epsilon}f(x) = \be[f(N_{\epsilon}(x))]$.
The noise operator has a convenient representation as well: for any $\epsilon > 0$, we have $N_{\epsilon} f = \sum_{|S|} (1-\epsilon)^{|S|} \hat f(S) \chi_S$.

A Boolean function $f:\{0,1\}^n \rightarrow \{0,1\}$ is called \emph{noise sensitive} if flipping each of its input bits with a small probability affects its output `significantly', i.e., if $\pr_{x^{(b)} \sim_{\eps} y^{(b)}} \lbs f(x^{(b)}) \neq f(y^{(b)}) \rbs = \Theta(\mathbb{E}[f])$. The relation between noise sensitivity and the Fourier expansion of the function was first established by Benjamini, Kalai, and Schramm in their classical paper~\cite{BKS99}. A central result of~\cite{BKS99} (specifically,~\cite[Theorem~1.9]{BKS99}) asserts that functions with a low Fourier weight on the low levels are noise sensitive.

The main application of~\cite{BKS99} was to show that various instances of \emph{percolation} are noise sensitive. In another classical paper, which was the first to show noise sensitivity of \emph{dynamic percolation}, Schramm and Steif~\cite{SS10} showed that any Boolean function that can be evaluated by a randomized algorithm which queries each input bit with a `small' probability, must have a small Fourier weight on the low levels, and thus, must be noise sensitive. Specifically, Schramm and Steif proved (\cite[Theorem~1.8]{SS10}):
\begin{theorem}\label{thm:SS}
Let $f:\{0,1\}^n \rightarrow \mathbb{R}$ be a function. Suppose that there is a randomized algorithm $A$ for determining the value of $f$ which examines some of the input bits of $f$ one by one, where the choice of the next bit examined may depend on the bits examined so far. Let $J \subset [n]$ be the (random) set of bits examined by the algorithm. Set $\gamma = \max_{i \in [i]} \Pr[i \in J]$. Then for any $k>0$, we have $W^k(f) \leq \gamma k \var(f)$.
\end{theorem}
Noise sensitivity and its relation to discrete Fourier analysis was studied extensively in the last two decades, and led to applications in theoretical computer science, probability theory, social choice theory and other fields (see the survey~\cite{Kalai18}). In particular, Schramm and Steif suggested (\cite[p.~623]{SS10}) that Theorem~\ref{thm:SS} may have applications in theoretical computer science.

We obtain such an application by using it to obtain our lower bound. While at a first glance, it is not clear how Theorem~\ref{thm:SS} is related to the noisy LPHS problem, it turns out we can reduce our problem into the setting of Theorem~\ref{thm:SS}, as will be shown below.

\subsection{Proof of Proposition~\ref{prop:lower}}

Using a series of reductions and Theorem~\ref{thm:SS}, we prove the following
% slightly stronger % OHAD: it is equivalent
result, which clearly implies Proposition~\ref{prop:lower}, since in our setting, the LPHS $h$ is a decision tree of depth $d$, and moreover, a noisy LPHS which is effective for a shift of $1$ is also effective for a shift of $0$, by a union bound.
\begin{proposition}\label{prop:noisy-lower1}
Let $\func{f,g}{\zo^{n}}{\zo}$ be binary decision trees of depth $d$, and suppose $\Omega(1) \leq \be[f], \be[g] \leq 1-\Omega(1)$. Then,
\begin{equation}\label{Eq:Lower-Aux1}
	\be_{r \sim \zo} \lbs \pr_{x\sim_{\eps} y}\lbs f(x) \neq g(y \ll r) \rbs \rbs \geq \Omega(\eps^{2/3}/d^{1/3}).
\end{equation}
\end{proposition}
Note that the assertion~\eqref{Eq:Lower-Aux1} is equivalent to
\begin{equation}\label{Eq:Lower-Aux2}
	4\be_{r \sim \zo} \lbs \cov\lbr f, N_{\eps} g_{\ll 1} \rbr \rbs \leq 1- \Omega(\eps^{2/3}/d^{1/3}),
\end{equation}
where $g_{\ll r}(y) = g(y \ll r)$ and $N_{\eps}$ is the noise operator. One can see this by computing
\begin{equation*}
\begin{split}
	4\cov\lbr f, N_{\eps} g_{\ll r} \rbr
	&= \cov\lbr 2f-1, N_{\eps} (2g_{\ll r}-1) \rbr \\
	&= \pr_{x}\lbs f(x) = g_{\ll r}(N_{\eps}(x)) \rbs - \pr_{x}\lbs f(x)\neq g_{\ll r}(N_{\eps}(x)) \rbs \\
	&= 1 - 2\pr_{x}\lbs f(x)\neq g_{\ll r}(N_{\eps}(x)) \rbs.
\end{split}
\end{equation*}

\medskip Our first reduction replaces $y \ll 1$ by an average over shifts $y \ll r$, where $r \in [0,R]$ is chosen uniformly at random. Namely, we claim that Proposition~\ref{prop:noisy-lower1} is easily implied by the following:
\begin{proposition}\label{prop:noisy-lower2}
Let $\func{f,g}{\zo^{n}}{\zo}$ be decision trees of depth $d$. Let $\epsilon>0$, $R=(d/\eps^2)^{1/3}$ and $k=1/(9R\eps)$. Then
\begin{equation}\label{Eq:Lower-Aux3}
	4\cov\lbr f, \be_{r\sim U(0, R)}[N_{1/k}g_{\ll r}] \rbr \leq 1-\Omega(1).
\end{equation}
\end{proposition}
Roughly speaking, the reduction follows by looking at the $R$ functions $\{g_{\ll \ell}\}_{\ell \in [R]}$, assuming on the contrary that~\eqref{Eq:Lower-Aux2} fails, applying its converse to deduce the pairs $(g_{\ll \ell}, N_{99\epsilon} g_{\ll \ell+1})$ are $1/(9R)$ close in $L_{2}$-norm, and using the triangle inequality to deduce that~\eqref{Eq:Lower-Aux3} fails as well, which is a contradiction. The formal argument is very similar to that of~\cite[Lemma~13]{DKK18}, and thus is omitted.

\medskip Our second reduction uses the noise to eliminate high-level Fourier coefficients of $N_{1/k}g$. We observe that as $N_{1/k} g = \sum_{|S|} (1-1/k)^{|S|} \hat g(S) \chi_S$, all Fourier coefficients of $N_{1/k} g$ above level $Ck$ for a sufficiently large constant $C$ are negligible (their sum of squares $\leq e^{-C}$), and would not asymptotically affect the validity of~\eqref{Eq:Lower-Aux3}. Hence, we can replace $N_{1/k}g$ with a truncation of its Fourier expansion into its first $Ck$ levels, i.e., $\sum_{|S| \leq Ck} \wh{N_{1/k}g}(S) \chi_S$. Note that the resulting function is not guaranteed to be Boolean anymore; we can only say that its variance is still at most 1, since for any $f$ we have $\var(f)=\sum_{S \neq \emptyset} \wh f(S)^2$ by Plancherel's identity~\eqref{Eq:Lower-Aux0}, and so truncation of the Fourier expansion cannot increase the variance. Therefore, Proposition~\ref{prop:noisy-lower2} is implied by the following.
\begin{proposition}\label{prop:noisy-lower3}
Let $\func{f}{\zo^{n}}{\zo}$ be a decision tree of depth $d$. Let $R=(d/\eps^2)^{1/3}$ and $k=1/(R\eps)$. Let $\func{\wt{g}}{\zo^{n}}{\reals}$ be a function with $\var(\wt{g})\leq 1$, which satisfies $\forall c\colon W^{>ck}(\wt{g}) \leq \exp(-c)$ and $|\wt{g}|\leq 1$. Then,
\begin{equation}\label{eq:main}
4\cov\lbr f, \be_{r\sim U(0, R)}(\wt{g}_{\ll r}) \rbr \leq 1- \Omega(1).
\end{equation}
\end{proposition}

\medskip Our third reduction moves the `smoothing' from $\wt{g}$ to $f$. Namely, we use the fact that it is clear by symmetry that~\eqref{eq:main} is equivalent to:
\begin{equation}\label{eq:main2}
4\cov\lbr \wt{g}, \be_{r\sim U(0, R)}(f_{\gg r}) \rbr \leq 1-\Omega(1).
\end{equation}
We claim that Proposition~\ref{prop:noisy-lower3} follows from the following relative of Theorem~\ref{thm:SS}, whose proof is similar to the ones of~\ref{thm:SS}. For the sake of completeness, we repeat it in Appendix~\ref{app:lower-noisy}.
\begin{lemma}\label{lem:SS}
	Let $f_{r}\colon \zo^{n} \to \zo$ be decision trees of depth $d$. Suppose that for every $i$ the probability $x_i$ is queried by the evaluation of $f_{r}$ on $x$ is $\leq \gamma$, where $x\sim\zo^{n}$ is uniformly distributed, and $r\sim R$ is distributed according to some specified distribution $R$.
	Then for any $k \in \pintegers$, the function $h(x)=\be_{r\sim R}[f_{r}(x)]$ satisfies
	$
		W^{k}(h) \leq \gamma k.
	$
\end{lemma}

% Ohad: Nathan, I think this is not better than the proof itself, sorry.
%First, we give an intuitive explanation. Let $h:= \be_{r\sim U(0, R)}(f_{\gg r})$. We can view $h$ as an evaluation of a function by a randomized algorithm. Since the function $f$ we begin with is a decision tree of depth $d$, the probability that each specific coordinate is queried in the `randomized algorithm' is low. Hence, Theorem~\ref{thm:SS} implies that the Fourier weight of $h$ on the low levels is low. On the other hand, the Fourier weight of $\wt{g}$ on the high levels vanishes, and hence, Plancherel's identity implies that $\cov(\wt{g},h)$ is small, thus implying~\eqref{eq:main2}. On an even more intuitive level, Theorem~\ref{thm:SS} implies that $h$ is noise sensitive; hence, when we consider its correlation with a noisy version of the original function $f$, the noise affects the result severely, and hence, the covariance is small.

%\medskip \noindent Let us present the formal proof.

\begin{proof}[Proof of Proposition~\ref{prop:noisy-lower3}]
Observe that the function $h=\be_{r\sim U(0,R)}(f_{\gg r})$ satisfies the assumptions of Lemma~\ref{lem:SS} with $\gamma = d/R$. This is because the probability $x_{i}$ is accessed by a random $f_{\gg r}$ with $r\sim U(0,R)$ equals to the probability a random coordinate $j\sim U(i, i+R)$ is accessed by $f$ -- and as $f$ accesses at most $d$ coordinates, this is upper bounded by $\gamma=d/R$. Hence, the theorem implies that for any $k>0$ we have $W^k(h) \leq \gamma k$. We deduce
\[
\sum_{0<|S|\leq Ck} \hat h(S)^2 \leq \gamma (Ck)^2 \var(h) \leq \gamma (Ck)^2/4.
\]
Since by assumption, the Fourier weight of $\wt{g}$ above the $Ck$-th level is $\leq e^{-C}$, Plancherel's identity and Cauchy-Schwarz inequality imply
\begin{equation}\label{eq:noisy-final}
\begin{aligned}
	4\cov(h,\wt{g})
	&= 4\sum_{S \neq \emptyset} \hat h(S) \wh{\wt{g}}(S)
	\leq 4\sum_{0<|S|\leq Ck} \wh{h}(S) \wh{\wt{g}}(S) + 4\sum_{Ck\leq |S|} \wh{h}(S) \wh{\wt{g}}(S) \\
	&\leq 4\sqrt{\sum_{0<|S|\leq Ck} \wh{h}(S)^2} \sqrt{\sum_{0<|S|\leq Ck} \wh{\wt{g}}(S)^2} + 4e^{-C/2}\\
	&\leq \sqrt{(Ck)^{2}\gamma} + 4e^{-C/2}
	= Ck\sqrt{d/R} + 4e^{-C/2}
 	\leq 0.9,
\end{aligned}
\end{equation}
where the last equality just substitutes the values of $k,d,R$ and $C=5$. This shows that~\eqref{eq:main2} holds, completing the proof.
\end{proof}

\subsection{A conjectured tight bound}

In~\cite[p.~623]{SS10}, Schramm and Steif conjectured a strengthening of Theorem~\ref{thm:SS}.
% \begin{conjecture}[SS10]\label{conj:SS}
% Let $f:\{0,1\}^n \rightarrow \mathbb{R}$ be a function. Suppose that there is a randomized algorithm $A$ for determining the value of $f$ which examines some of the input bits of $f$ one by one, where the choice of the next bit examined may depend on the bits examined so far. Let $J \subset [n]$ be the (random) set of bits examined by the algorithm. Set $\gamma = \max_{i \in [i]} \Pr[i \in J]$. Then for any $k>0$, we have
% \[
% \sum_{0<|S|\leq k} \hat f(S)^2 \leq \gamma k \var(f).
% \]
% \end{conjecture}
\begin{conjecture}[SS10]\label{conj:SS}
In the setting of Theorem~\ref{thm:SS}, one has
$
\sum_{0<|S|\leq k} \widehat{f}(S)^2 \leq \gamma k \var(f).
$
\end{conjecture}
We make the following evidently related conjecture
\begin{conjecture}\label{conj:SS2}
In the setting of Lemma~\ref{lem:SS}, one has
$
\sum_{0<|S|\leq k} \widehat{h}(S)^2 \leq \gamma k.
$
\end{conjecture}

By applying the same reductions as above and replacing the bound of Lemma~\ref{lem:SS} with that of Conjecture~\ref{conj:SS2}, the following conjecture is implied.
\begin{conjecture}\label{conj:noisy-lower1}
Let $\func{f,g}{\spm^{n}}{\zo}$ be binary decision trees of depth $d$, and suppose $\Omega(1) \leq \be[f], \be[g] \leq 1-\Omega(1)$. Then,
\begin{equation}\label{Eq:Conj-Lower-Aux1}
	\pr_{x\sim_{\eps} y}\lbs f(x) \neq g(y \ll 1) \rbs \geq \Omega(\sqrt{\eps/d}).
\end{equation}
\end{conjecture}
This conjectured lower bound matches the error probability we obtain in our algorithm up to polylogarithmic factors. Hence, we conclude that our noisy LPHS algorithm obtains the optimal error rate (up to polylogarithmic factors) for all ranges of $\eps$, if we assume Conjecture~\ref{conj:SS2} which is a variant of Schramm and Steif's Conjecture~\ref{conj:SS}.
%\ynote{Optimal up to polylogarithmic factors?}

\subsection{Ruling out sublinear noisy LPHS for big shifts}
In light of Theorem~\ref{th-main} and Lemma~\ref{lem:shift}, there is a shift-bounded, non-cyclic $(n, b=1, d, \delta, R)$-LPHS $h$ with $d=\wt{O}(\sqrt{n})$, $\delta = o(1)$ and $R=O(n)$. That is, $h$ makes only $d$ queries to its input, and yet $\pr_{r\sim U(1, R)}[h(x) \neq h(x \lll r) + r] \leq \delta$. What happens when we add noise in this context? Is there a sublinear LPHS which is resilient to constant (say, $\eps=0.001$) noise? We answer this question negatively.
\begin{corollary}\label{cor:inexistence}
	Any noise-resilient, shift-bounded $(n, b=1, d, \delta, \eps, R)$-LPHS with $\delta \leq 1/3$ has $d > \Omega(R \eps^2)$.
\end{corollary}

We note that while the simple restriction $\delta \geq \Omega(\epsilon)$ (following from~\cite[Lemma~2.2]{MosselO05} and Lemma~\ref{lem-smoothness}) easily rules out the existence of LPHS with $\delta \geq \Omega(\eps)$, it does not rule out an LPHS with $\delta < \Omega(\eps)$. For this purpose, the proof of Corollary~\ref{cor:inexistence} uses a variant of Proposition~\ref{prop:noisy-lower2}, and appears in Appendix~\ref{app:lower-noisy}.

\medskip \noindent Several extensions of the results presented in this section are discussed in Appendix~\ref{app:lower-noisy}.

%\section{Lower bounds for $d^{-3} \leq \eps \leq d^{-1}$}
%\label{sec:lower}
%
%In this section we prove the remaining non-trivial part of Theorem~\ref{thm:lower}, namely, that any $(n,1,d,\eps,\delta)$-LPHS for $d^{-3} \leq \eps \leq d^{-1}$ satisfies $\delta \geq \eps^{2/3}/d^{1/3}$. Yet, we believe that the true lower bound is $\sqrt{\eps/d}$. This is formalized in Conjecture~\ref{conj:main}. It is stated for functions $f,g$ with a domain of $\spm^{n}$ and a binary range, but it is easy to verify that this conjecture implies the optimality (up to logarithmic factors) of the third upper bound derived in Theorem~\ref{thm:algs}.
%
%\begin{conjecture}\label{conj:main}
%Let $\func{f,g}{\spm^{n}}{\zo}$ be binary decision trees of depth $d$, and suppose $\Omega(1) \leq \be[f], \be[g] \leq 1-\Omega(1)$. Then,
%\[
%	\pr_{x\sim_{\eps} y}\lbs f(x) \neq g(y \ll 1) \rbs \geq \sqrt{\eps/d}.
%\]
%
%\end{conjecture}
%Notice that when $\epsilon > 1/d$ or $\epsilon < 1/d^{3}$, we already know better bounds: $\epsilon, 1/d^{2}$ respectively.
%
%Using the usual triangle-inequality + coupling argument along smearing of length $R=\sqrt{d/\eps}$, Conjecture~\ref{conj:main} is implied from
%\begin{conjecture}\label{conj:main2}
%Let $\func{f,g}{\spm^{n}}{\zo}$ be decision trees of depth $d$. Let $R=\sqrt{d/\eps}$ and $k=1/(R\eps)$. Then
%\[
%	\cov\lbr f, \be_{r\sim U(0, R)}[N_{1/k}g_{\ll r}] \rbr \leq 1-\Omega(1).
%\]
%\end{conjecture}
%Notice that in the previous conjecture $N_{1/k}g$ may be replaced by $\func{h}{\spm^{n}}{\reals}$ with degree $O(k)$ and $\var(h) \leq 1$. This is because the Fourier weight of $h$ above level, say, $3k$ is negligible, and would not asymptotically affect the $\Omega(1)$. The loss in this relaxation is that now $h$ might not be bounded by $1$. Let us put this in a new conjecture.
%
%\begin{conjecture}\label{conj:main3}
%Let $\func{f}{\spm^{n}}{\zo}$ be a decision tree of depth $d$. Let $\func{g}{\spm^{n}}{\reals}$ be a function with $\var(g)\leq 1$, which is either of degree $k$, or satisfies $\forall c\colon W^{>ck}(g) \leq \exp(-c)$ and $|g|\leq 1$. Then,
%\begin{equation}\label{eq:main}
%\cov\lbr f, \be_{r\sim U(0, R)}(g_{\ll r}) \rbr \leq O\lbr \sqrt{dk/R}\rbr.
%\end{equation}
%\end{conjecture}
%We note the there are examples that show that this bound cannot be improved as a function of $d,k,R$ for many interesting values of $d,k,R$ (of course, our algorithm is such an example, but it only applies to $dk/R \sim 1$, which does not determine the correct exponent).
%This makes things more intricate, as we cannot apply arguments such as the ones used in~\cite{DKK18} to obtain lower bounds with no noise.
%
%Notice also that $f$ may be replaced by $\be_{r\sim U(R)} [f_{\ll r}]$, as this just doubles the randomization in the shift between the two functions. Also, conveniently, further shifting schemes are possible.
%
%\subsection{Argument based on \cite{SS05}}
%Applying a standard Cauchy-Schwarz to~\eqref{eq:main}, we are left with proving
%\begin{conjecture}\label{conj:main4}
%Let $f,g$ be as in Conjecture~\ref{conj:main3}. Let $J$ be the random-variable indicating the indices of the bits queried by the decision tree $f$, applied on a random string $x$. Similarly, denote $g_{J}$ to be the function with the values of (the implicit) $x$ substituted at indices $J$. Then,
%\[
%	\be_{x,J}\lbs \lbr\be_{r\sim U(R)}[g_{\ll r}]_{J}\rbr^{2} \rbs \leq dk/R.
%\]
%\end{conjecture}
%
%Schramm and Steif already conjectured an almost equivalent conjecture a long ago~\cite{SS05}. (The paper in which the conjecture was stated is very well-known in the probability community; it deals with dynamic percolation.)
%\begin{conjecture}[SS05 conjecture]\label{conj:schramm}
%Let $\func{f_{r}}{\spm^{n}}{\zo}$ be decision trees of depth $d$. Suppose that upon drawing the input $x$ and a decision tree $f_{r}$ at random, the probability that a single coordinate $x_{i}$ is queried, is always bounded by $\gamma$. Then,
%\[
%W^{\leq k}(\be_{r}[f_{r}])-\wh{f}(\es)^{2} \leq k\gamma.
%\]
%\end{conjecture}
%In our case, notice $\gamma = d/R$.
%Short of proving this, they managed to prove
%\begin{theorem}[\cite{SS05}]\label{thm:ss05_bound}
%Under the assumptions in Conjecture~\ref{conj:schramm}, we have for all $k>0$,
%\[
%	W^{=k}\lbr \be_{r}[f_{r}] \rbr \leq k \gamma,
%\]
%and hence $W^{\leq k}\lbr \be_{r}[f_{r}] \rbr - \wh{f}(\es)^{2} \leq k^{2} \gamma$.
%\end{theorem}
%
%Before repeating their proof, let us see what it implies about our problem.
%
%\begin{lemma}
%Let $f,g,k,d,R$ be as in Conjecture~\ref{conj:main3}. Then,
%\[
%	\cov\lbr f, \be_{r\sim U(R)}(g_{\ll r})\rbr \leq O(k\sqrt{d/R})
%\]
%\end{lemma}
%\begin{proof}
%The expression we would like to bound equals
%\[
%	\cov\lbr \be_{r\sim U(R)}(f_{\gg r}), g\rbr.
%\]
%However, $h=\be_{r\sim U(R)}(f_{\gg r})$ satisfies the assumptions of Theorem~\ref{thm:ss05_bound} with $\gamma = d/R$. Hence, $W^{\leq k}(h)-\wh{h}(\es)^{2} \leq k^{2}\gamma$. Since $g$ is, by assumption, of degree $k$ (or something similar), then by Cauchy-Schwarz
%\[
%	\cov(h,g) \leq \sqrt{W^{\leq k}(h)-\wh{h}(\es)^{2}} \cdot \sqrt{\be[g^{2}]} \leq \sqrt{k^{2}\gamma} \leq k\sqrt{d/R}.
%\]
%\end{proof}
%
%Let us peel this information off, and understand the consequences regarding Conjecture~\ref{conj:main}. Recall we wish our bound of $k\sqrt{d/R}$ to be $1-\Omega(1)$. That is $k^{2}\sim R/d$. Recall the interesting bound in Conjecture~\ref{conj:main} equals $1/R$ and that $k$ is defined to satisfy $kR\eps = 1$. Putting this together we conclude $1/(R\eps)^{2} \sim R/d$, that is $R^{3} \sim d/\eps^{2}$. Since our bound of interest is $1/R$, we conclude with a nontrivial bound of $\eps^{2/3}/d^{1/3}$.

%\begin{proof}[Proof of Theorem~\ref{thm:ss05_bound}]
%Let $f=\be_{r}[f_{r}]$, and denote $g=f^{=k}$. Notice $W^{=k}(f)=\be[fg]$. Let $J$ be the set of coordinates queried by the natural algorithm corresponding to $f$ -- draw $r$, and draw the value of the relevant coordinate, depending on the structure of $f_{r}$ and previous queries. Similarly, let $x_{J}$ be the values of these queried coordinates.
%\[
%\be[fg] \underbrace{\leq}_{\mrm{total\ probability}} \be_{J,x_{J}}\lbs \be\lbs \given{f\cdot g}{J,x_{J}} \rbs \rbs \leq \be_{J,x_{J}}\lbs  f \cdot\be\lbs \given{g}{J,x_{J}} \rbs \rbs
%\]
%Applying Cauchy-Schwarz,
%\[
%\leq \sqrt{\be[f^{2}]} \cdot \sqrt{\be_{J,x_{J}}\lbs \be\lbs \given{g}{J,x_{J}} \rbs^{2} \rbs} \leq \sqrt{\be_{J, x_{J}}[g_{J}^2]},
%\]
%where $g_{J}$ is the function obtained by substituting the value of $x_{J}$, and $g_{J}^{2}\in \reals$ is a shorthand for $\be[g_{J}(x)^{2}]=\wh{g_{J}}(\es)^{2}$.
%
%To upper bound $\be_{J}[g_{J}^{2}]$, recall that $g$ is homogenuous of degree $k$. Notice that always, regardless of $J$ and $x_{J}$, we have $\wh{g_{J}}(\es)^{2}+\sum_{|S|=k}\wh{g_{J}}(S)^{2} \leq \be[g^2]$.
%
%However, $\wh{g_J}(S)=\wh{g}(S)\cdot \one\{J\cap S=\es\}$; hence, $\be_{J}[\wh{g_J}(S)^{2}]\geq \wh{g}(S)^{2}(1-k\gamma)$.
%
%Overall $\wh{g_{J}}(\es)^{2}\leq \be[g^{2}]-\sum_{S \neq \es} \wh{g}(S)^{2}(1-k\gamma) \leq k\gamma \var(g)$, using that $g$ is homogenous of degree $k$.
%In total,
%\[
%	W^{=k}(f) = \be[fg] \leq \sqrt{k\gamma W^{=k}(f)}.
%\]
%\end{proof}



==> Overview.tex <==
% !TEX root = ../LPHS.tex


\section{Overview of Techniques}

We summarize our main technical results regarding the noise-resilient and multi-dimensional LPHS variants. In all theorems stated below, the $\tilde{\Omega}$ and $\tilde{O}$ hide a poly-logarithmic factor in $n$.

%\ynote{ For algorithmic applications, one may care about combinations of different modifiers from Definition~\ref{def-lphs}. For instance, what can we say about noise-resilient 2D-LPHS? And how does the worst-case variant from Appendix~\ref{sec-worstcase} carry over to the 2D, noise-resilient, and/or non-cyclic modifiers?}

%\subsection{LPHS from Distributed Discrete Logarithm}

As discussed, we begin by demonstrating an equivalence between our basic notion of LPHS and a particular form of the cryptographic notion of a distributed discrete log (DDL) algorithm that functions within the generic group model (see Section~\ref{sec:relations}). As such, we obtain LPHS constructions with sublinear query complexity, leveraging the recent results on DDL from~\cite{BGI16,DKK18}.

In what follows, we expand on our results on noise-resilient LPHS and 2-dimensional LPHS.


%\subsection{One-Dimensional Noise-Resilient LPHS}
\subsection{Noise-Resilient LPHS}

Recall that in the noise-resilient variant,
%the problem is one-dimensional (as in~\cite{DKK18}), but in addition to the shift between the inputs,
the LPHS has to overcome random noise which flips each bit of one of the inputs with probability $\eps$.
%\ynote{What can we say about a {\em worst-case} error, flipping arbitrary $\eps n$ bits?}

For this problem, we present an algorithm and show that it is essentially optimal if we assume a well-known conjecture of Schramm and Steif~\cite{SS10} on noise sensitivity of certain Boolean functions; we also obtain a somewhat weaker unconditional lower bound, using a theorem
%of Schramm and Steif
from~\cite{SS10}.

More specifically, on the upper bound side we have the following result.
\begin{theorem}
\label{thm:1dupper}
For $n = \tilde{\Omega}(d^2)$, there is an $(n,1,d,\eps,\delta)$-LPHS that satisfies
\[
    \delta =
\begin{dcases}
    \tilde{O}(1/d^2),& \eps \leq d^{-3}\\
    \tilde{O}(\eps),         & \eps \geq d^{-1}\\
	\tilde{O}(\sqrt{\eps/d}), &  d^{-3} \leq \eps \leq d^{-1}.\\
\end{dcases}
\]
There is also a non-cyclic LPHS with the same parameters.
\end{theorem}
For $\eps \geq d^{-1}$, the upper bound is attained by the simple MinHash algorithm (i.e., the algorithm of~\cite{BGI16} for the DDL problem described in the Introduction), and for $\eps \leq d^{-3}$, the upper bound is attained by the Iterated Random Walk (IRW) algorithm of~\cite{DKK18} (see Appendix~\ref{app:dkk}). The range $d^{-3} \leq \eps \leq d^{-1}$ is more interesting. For $\eps$ in this range, the upper bound is attained by a mixture between the MinHash and the IRW algorithms: an algorithm that (for appropriately chosen $T_1,T_2$ with $T_1 \cdot T_2 = d$) applies IRW with $d'=T_2$ steps on blocks of size $T_1$, where after each step, it applies MinHash on the block in which the walk is located. This algorithm was also presented in~\cite{DKK18} (specifically, in Appendix~D.2), but for a different purpose of preserving locality of queries.

\medskip On the lower bound side we obtain the following unconditional result.
%We summarize our results on LPHS in one dimension. The following theorem establishes lower bounds and is proved in Section~\ref{??}.
\begin{theorem}
\label{thm:1dlower}
For $n = \Omega(d^2)$, any (cyclic or non-cyclic) $(n,1,d,\eps,\delta)$-LPHS satisfies
    $$\delta \geq \max(\Omega(1/d^2), \Omega(\eps), \eps^{2/3}/d^{1/3}).$$
\end{theorem}
That is, in the ranges $\eps \geq d^{-1}$ and $\eps \leq d^{-3}$, Theorem~\ref{thm:1dupper} is tight, while for $d^{-3} \leq \eps \leq d^{-1}$, there is some gap between our upper and lower bounds. The proof of Theorem~\ref{thm:1dlower} in this case uses a seemingly unrelated well-known result of Schramm and Steif~\cite{SS10} on noise sensitivity of Boolean functions. Specifically, Schramm and Steif proved that if some Boolean function can be evaluated by a randomized algorithm that queries each input bit with only a small probability, then it must be noise sensitive, and more precisely, most of the weight in its Fourier expansion must lie on the `high levels' (a detailed explanation is given in Section~\ref{sec:lower-noisy}). We show that our noisy LPHS problem can be reduced into a variant of the setting considered by Schramm and Steif, and so their result can be used to show that the correlation between $f(x)$ and $g(y \ll 1)+1$ is sensitive to noise, thus yielding a lower bound on the error for any fixed noise rate $\eps$. The proof uses discrete Fourier analysis, and more specifically, the convenient representations of correlation, low number of queries, and noise, as properties of the Fourier expansion of the underlying Boolean functions.

In their paper~\cite{SS10} (which is well-known mostly in the probability community, due to its fundamental contribution to the study of percolation), Schramm and Steif also conjectured that a stronger variant of their aforemention theorem holds.
We show that assuming a closely related variant of this conjecture, our upper bound is essentially tight, up to logarithmic factors.

 %
%
%
%The following theorem establishes upper bounds. We sketch its proof in Section~\ref{sec:dkk}. However, we note that this algorithm is based on an algorithm presented in~\cite{DKK18}, which was designed for a different purpose (of preserving locality of queries). Hence, it is not among the main technical contributions of the paper.
%\begin{theorem}
%\label{thm:1dupper}
%For $n = \tilde{\Omega}(d^2)$, there is an $(n,1,d,\eps,\delta)$-LPHS that satisfies
%\[
%    \delta =
%\begin{dcases}
%    \tilde{O}(1/d^2),& \eps \leq d^{-3}\\
%    \tilde{O}(\eps),         & \eps \geq d^{-1}\\
%	\tilde{O}(\sqrt{\eps/d}), &  d^{-3} \leq \eps \leq d^{-1}.\\
%\end{dcases}
%\]
%There is also a non-cyclic LPHS with the same parameters.
%\end{theorem}
%
%Therefore, the upper bounds for $\eps \leq d^{-3}$ and $\eps \geq d^{-1}$ established in Theorem~\ref{thm:algs} are tight up to logarithmic factors in $d$.
%
%We also conjecture that the upper bound of $\tilde{O}(\sqrt{\eps/d})$ for $d^{-3} \leq \eps \leq d^{-1}$ is tight up to logarithmic factors. However, we cannot prove this and can only prove (in Section~\ref{sec:lower}) a weaker lower bound of $\delta \geq \eps^{2/3}/d^{1/3}$. Note that the weaker lower bound is tight in the region where $\eps \sim 1/d$. However, in the case where $\eps \sim 1/d^{3}$ we only get a lower bound of $1/d^{7/3}$, instead of $1/d^{2}$. The crossover point is $\eps \sim d^{-5/2}$, from which we cannot prove a better bound than the trivial $1/d^{2}$.

\subsection{LPHS in Higher Dimensions}

We now provide an overview of our results for the $k$-dimensional variant of LPHS. Here we focus mainly on the 2-dimensional case, in which the input is arranged in a square, and the LPHS algorithm has to accommodate shifts on both axes.

The simple MinHash algorithm can be applied in this setting as well, leading to error probability of $1/\sqrt{d}$, where $d$ is the number of queries. A more promising algorithm is applying some combination of 1-dimensional IRW algorithms on both axes independently. While such an algorithm is indeed more efficient, it still leads to an error probability of $O(d^{-4/5})$. We obtain the following stronger result:
\begin{theorem} \label{thm:2dupper}
For $n = \tilde{\Omega}(d^2)$ and any $b > 0$, there is a 2-dimensional $(n,b,d,\delta)$-LPHS that satisfies $\delta = \tilde{O}(d^{-7/8})$. There is also a non-cyclic 2-dimensional LPHS with the same parameters.
\end{theorem}
This upper bound is obtained via a
%rather complex
specialized 3-stage algorithm (see Appendix~\ref{app:2D78}) that does not use 1-dimensional IRW as a subroutine.

\medskip \noindent On the lower bound side, we prove:
\begin{theorem} \label{thm:kdlower}
For $n = \Omega(d^2)$ and any $b > 0$, every $k$-dimensional (cyclic or non-cyclic) $(n,b,d,\delta)$-LPHS satisfies $\delta = \Omega(d^{-2/k})$.
\end{theorem}
The proof
%is a somewhat complex
of this lower bound is based on a rather delicate argument involving Minkowski sums and differences of sets in $\mathbb{R}^k$.

\medskip \noindent In addition, we present another 2-dimensional LPHS algorithm, which is much harder to analyze, but for which we conjecture that the error rate is at most $\tilde{O}(d^{-1})$, which is essentially tight by Theorem~\ref{thm:kdlower}.
%\ynote{ Maybe say something here about the evidence for the conjecture. Are the independence assumptions empirically validated? }
%
%Hence, for $k=2$ dimensions, there is a gap between our upper and lower bounds. We also have a 2-dimensional LPHS that we conjecture to satisfy $\delta = \tilde{O}(d^{-1})$ (which is optimal up to logarithmic factors), yet we cannot formally analyze its error probability.

\iffalse
\subsection{LPHS with Preprocessing}

We use the recent
%breakthrough
result of Corrigan-Gibbs and Kogan~\cite{Corrigan-GibbsK18} on the discrete logarithm problem with preprocessing to prove the following theorem, which asserts that preprocessing ability cannot be used to significantly decrease the error probability of the LPHS algorithm.
\begin{theorem} \label{thm:prelower}
For $n = \tilde{\Omega}(d^2 \cdot \alpha)$, any (cyclic or non-cyclic) $(n,1,d,\delta)$-LPHS that receives an advice string of length $\alpha$, satisfies $\delta = \tilde{\Omega}(d^{-2} \cdot \alpha^{-1})$.
\end{theorem}

\fi


==> SetSimilarity.tex <==

\section{Set-Similarity}
\label{app:setsim}

In this section we show that if one replaces ``shift distance'' by ``set similarity,'' then there are {\em no} sublinear sketching algorithms (with $d = n^{\alpha}$ for $\alpha < 1$) that have polylogarithmic sketch size.

The set-similarity problem can be described as a simultaneous communication game between parties $\mathcal{A}$, $\mathcal{B}$ and $\mathcal{C}$. The input space is an ordered set containing $n$ strings of length $b$ bits. We assume that $b = \log^2 n$, although we will not explicitly use this in the analysis. The distance between two such sets is (half) the number of strings appearing in exactly one of them.

The input of each of $\mathcal{A}$ and $\mathcal{B}$ consists of a set of $n$ uniform and independent strings of length $b$. At the beginning of the game, a bit $s \in \{0,1\}$ is chosen uniformly at random. If $s = 0$, then $\mathcal{A}$ and $\mathcal{B}$ receive identical sets, but the strings in each set appear in uniform and independent order. If $s = 1$, then the sets of $\mathcal{A}$ and $\mathcal{B}$ are chosen in the following way: $\mathcal{A}$'s set is chosen uniformly at random, while $\mathcal{B}$'s set is obtained from $\mathcal{A}$'s set by shuffling it uniformly at random and then picking a uniform subset of size $\alpha n$ (where $0 < \alpha \leq 1$ is a constant), and replacing it by $\alpha n$ fresh random strings. Each party ($\mathcal{A}$ and $\mathcal{B}$) makes $d$ queries to its set (a query to index $i \in [n]$ is answered by the string at that index) and sends a message (sketch) of size $c$ to party $\mathcal{C}$, whose goal is to determine $s$ (i.e., distinguish between a similarity of 1 and of $\approx (1 -\alpha) n$) with probability $2/3$ (or any constant probability bounded away from $1/2$).

We prove a lower bound of $c \cdot d = \Omega(n)$ for the problem, which holds (even) for $\alpha = 1$. This implies that if we restrict the sketch size $c$ to be poly-logarithmic in $n$, then the number of queries $d$ needs to be (almost) linear in order for $\mathcal{C}$ to succeed with the desired probability.

In fact, we will prove this lower bound for a more general 2-player communication game, where $\mathcal{A}$ is allowed to query each element of its set, and sends a sketch of size $c$ to $\mathcal{B}$ which tries to determine $s$ from $\mathcal{A}$'s message and its $d$ queries (it is easy to see that a lower bound for this game implies the same lower bound for the simultaneous communication game).

\begin{theorem}
\label{thm:setsim}
Suppose that $\mathcal{A}$ and $\mathcal{B}$ succeed with probability $2/3$ in the 2-player set-similarity communication game. Then $c \cdot d = \Omega(n)$.
\end{theorem}

A simple observation is that (regardless of $s$) the order of the elements in each input set is uniform and independent. Thus, the exact query set of $\mathcal{B}$ is insignificant and we may assume without loss of generality that $\mathcal{B}$ queries the first $d$ elements.

Let $S$ be a random variable for the bit $s$.
Denote by $X$ the random variable for the set of $\mathcal{A}$ and by $Y$ the random variable
for the ordered set of $d$ answers to the queries of $\mathcal{B}$.
Denote by $M$ a random variable for the message of $\mathcal{A}$.
let $T$ be a random variable for the query set of $\mathcal{B}$ with respect to the set of $\mathcal{A}$. For example, if $s=0$, then $T[1]$ is the index in $\mathcal{A}$'s set of the first element in $\mathcal{B}$'s set. Denote by $X[T]$ the answers to the query set $T$ with respect to $X$.
Note that if $s = 0$, then $X[T] = Y$, whereas if $s = 1$, they generally differ.
Denote by $\gamma$ the error probability of $\mathcal{B}$.

\begin{proof}

$\mathcal{B}$ predicts $s$ based on $\mathcal{A}$'s message and the answers to its queries,
and $s$ is uniform in $\{0,1\}$.
Therefore, Fano's inequality for a random variable of support size 2
implies that
$$\HH(\gamma) \geq \HH(S \mid M,Y).$$
Note that $\HH(S \mid M,Y) = \HH(S) - \I(S ; M,Y) = 1 - \I(S ; M,Y)$,
and thus we upper bound $\I(S ; M,Y)$

First, we have $$\I(S ; M,Y) \leq \I(M ; Y \mid S).$$
The proof is based on the equalities $I(S ; M) = 0$ and $I(S ; Y) = 0$. 
%It is very similar to the proof of Claim~\ref{clm:c1}, and we therefore omit it.

Next,
$$\I(M ; Y \mid S) = \frac{1}{2}(\I(M; Y \mid S = 0) + \I(M; Y \mid S = 1)).$$
Note that $\I(M; Y \mid S = 1) = 0$,
as conditioned on $S=1$, $X$ (and $M$) is independent of $Y$.
In addition,
$$\I(M; Y \mid S = 0) = \I(M; X[T] \mid S = 0).$$

Finally,
$$\I(M; X[T] \mid S = 0) \leq
\frac{d}{n} \cdot \HH(M) \leq
\frac{c\cdot d}{n}.
$$
%The proof of the first inequality is very similar to the proof of Claim~\ref{clm:c2} and we omit it. 
%The main observation required is that for every $i$, $\Pr[i \in T] \leq \frac{d}{n}.$
The first inequality follows from the fact that for every $i$, $\Pr[i \in T] \leq \frac{d}{n}$.

Overall, we obtain $$\I(S ; M,Y) \leq \frac{c \cdot d}{2n},$$ and
therefore, $$\HH(\gamma) \geq 1 - \frac{c \cdot d}{2n}.$$
Thus, if
$\gamma < \frac{1}{3}$, then $c \cdot d = \Omega(n)$ as claimed.

\end{proof}



